Memory Under Siege: A Comprehensive Survey of Side-Channel Attacks on Memory

Side-channel attacks on memory (SCAM) exploit unintended data leaks from memory subsystems to infer sensitive information, posing significant threats to system security. These attacks exploit vulnerabilities in memory access patterns, cache behaviors, and other microarchitectural features to bypass traditional security measures. The purpose of this research is to examine SCAM, classify various attack techniques, and evaluate existing defense mechanisms. It guides researchers and industry professionals in improving memory security and mitigating emerging threats. We begin by identifying the major vulnerabilities in the memory system that are frequently exploited in SCAM, such as cache timing, speculative execution, \textit{Rowhammer}, and other sophisticated approaches. Next, we outline a comprehensive taxonomy that systematically classifies these attacks based on their types, target systems, attack vectors, and adversarial capabilities required to execute them. In addition, we review the current landscape of mitigation strategies, emphasizing their strengths and limitations. This work aims to provide a comprehensive overview of memory-based side-channel attacks with the goal of providing significant insights for researchers and practitioners to better understand, detect, and mitigate SCAM risks.

==> Sections/Miscelleneous/Cryptographic_and_Algorithmic_Mitigations__CAM_.tex <==
\subsection{Cryptographic and Algorithmic Mitigations (CAM):} Cryptographic and algorithmic mitigations provide an essential layer of defense against memory side-channel attacks by redesigning protocols, cryptographic algorithms, and associated computations to resist side-channel leakage. These strategies ensure sensitive operations remain secure, even in adversarial environments, by eliminating or obfuscating leakage through timing, power, or memory access patterns. They provide a robust foundation for resisting diverse side-channel vulnerabilities.
One key approach involves leveraging cryptographic mechanisms to protect sensitive keys and data. Techniques leveraging hardware transactional memory ensure that sensitive cryptographic keys are shielded from potential leakage during execution. Execution path obfuscation disrupts digital side-channel analysis, closing timing-based attack vectors\cite{rane2015raccoon}. These approaches integrate seamlessly into protocols, offering robust security without significant performance trade-offs.
Algorithmic diversity also plays a crucial role in mitigating memory-based side-channel attacks. Blinding techniques, such as adding random noise to intermediate cryptographic computations or masking key-dependent operations in Elliptic Curve Cryptography (ECC), obscure leakage and reduce predictability for attackers\cite{kocher1996timing, goubin2002refined}. Memory polymorphism dynamically alters memory layouts to disrupt predictable patterns that attackers rely on \cite{jiang2020mempoline}. Combining code polymorphism and encryption protects software components, ensuring that side-channel attacks exploiting ciphertext leaks are rendered ineffective\cite{morel2023code}. Homomorphic encryption enables secure computations on encrypted data without decryption, minimizing adversarial exposure. For example, Practical Fully Homomorphic Encryption by \textit{Gentry et al.} showcases its utility for secure memory operations and distributed systems\cite{gentry2009fully}.
Addressing timing side-channel vulnerabilities remains a critical focus of cryptographic and algorithmic mitigations. Side-channel-free cryptographic primitives, such as the Montgomery ladder for RSA, prevent timing-based attacks by ensuring constant-time execution across operations\cite{joye2002montgomery}. Additionally, Targeted mitigations secure cryptographic computations, ensuring execution time remains independent of input values\cite{wichelmann2023cipherfix}. A systematic framework detects and repairs timing-based side-channel vulnerabilities in application code by addressing both known and emerging vulnerabilities, these approaches ensure resilience against evolving threats\cite{wu2018eliminating}.
Memory encryption and authentication further reinforce protection against memory side-channel attacks. Protocol redesign, such as modifying handshake protocols to eliminate timing-based leakage, complements encryption-based defenses\cite{dziembowski2008leakage}. \textit{Xiong et al.} safeguards memory against DPA attacks by combining fresh re-keying and authentication trees, limiting key usage, and employing plaintext masking for robust encryption and authentication\cite{unterluggauer2019meas}. Threshold cryptography, which splits cryptographic keys into shares, reduces single-point leakage risks, ensuring enhanced security in distributed systems. Addressing power-based leakages, optimized cryptographic code is secured to prevent adversarial exploitation\cite{tsoupidi2023securing}.
Cryptographic and algorithmic mitigations are essential in layered security strategies. As memory side-channel attacks evolve, these defenses must innovate to ensure robust protection while maintaining adaptability in modern computing environments.


==> Sections/Miscelleneous/Hardware_Level_Mitigations__HLM_.tex <==
\subsection{Hardware Level Mitigations (HLM):} Hardware Level Mitigations form the foundational layer of defense against memory side-channel attacks by addressing vulnerabilities intrinsic to physical architectures and microarchitectural components. These defenses are designed to counter adversaries who exploit timing variations, access patterns, or speculative execution flaws to extract sensitive information. As advanced techniques like \textit{Prime+Probe} and \textit{Rowhammer} continue to evolve, hardware-based solutions have become indispensable for safeguarding modern computing systems~\cite{liu2015last, mutlu2019rowhammer}.

A core focus of hardware mitigation is cache architecture. By redesigning how caches manage memory, systems can reduce timing discrepancies that side-channel attacks rely on. Partitioning techniques such as cache coloring enforce process isolation at the hardware level. \textit{Liu et al.} proposed dedicating specific cache sets to individual processes to prevent resource contention and reduce leakage in shared environments~\cite{liu2016catalyst}. \textit{Werner et al.} introduced dynamic cache set randomization, making it difficult for attackers to predict access patterns~\cite{werner2019scattercache}. To defend against speculative execution attacks, \textit{Kiriansky et al.} implemented strict cache isolation policies~\cite{kiriansky2018dawg}, while \textit{Gruss et al.} utilized hardware transactional memory to protect sensitive code paths by isolating execution states~\cite{gruss2017strong}. Additionally, \textit{Chen et al.} proposed dynamic cache flushing to periodically clear shared caches, thereby mitigating speculative traces and residual data leakage~\cite{chen2018racing}.

Beyond caches, memory-level technologies have advanced to prevent fault and access-based attacks. \textit{Rowhammer} resistant DRAM designs like target row refresh (TRR), \textit{PROTRR} monitor and regulate activation frequencies to prevent disturbance errors~\cite{frigo2020trrespass, marazzi2022protrr}. Error-Correcting Code (ECC) memory adds fault resilience by automatically detecting and correcting bit flips in adversarial scenarios~\cite{kim2023kill}. \textit{Kim et al.} introduced DRAM randomization, dynamically changing physical memory layouts to obscure timing-based patterns~\cite{kim2014flipping}. \textit{Dessouky et al.} combined static and dynamic cache configurations to balance performance and security in trusted platforms~\cite{dessouky2020hybcache}. Similarly, \textit{Godfrey et al.} proposed tenant isolation mechanisms in cloud environments to prevent cross-VM cache-based leakage~\cite{godfrey2014preventing}.

At the processor level, secure hardware design mitigates microarchitectural risk such as speculative leakage. Speculation barriers like \textit{SafeSpec}~\cite{khasawneh2019safespec} and \textit{PoisonIvy}~\cite{ lehman2016poisonivy} prevent transient instructions from leaving observable states. \textit{Yan et al.} developed \textit{InvisiSpec}~\cite{yan2018invisispec} to suppress speculative execution traces from becoming accessible to attackers. Secure enclave extensions, such as enhanced SGX designs, strengthen defenses against controlled-channel attacks by hiding memory access patterns~\cite{shih2017t}. \textit{Van Bulck et al.} introduced architectural separations between privileged and non-privileged modes to limit leakage across protection domains~\cite{van2018foreshadow}.

Despite trade-offs in cost and performance, hardware-level mitigations provide a robust root of trust against side-channel attacks. By embedding protection directly into the architecture, they ensure long-term resilience against evolving consumer and cloud system threats.

==> Sections/Miscelleneous/Isolation_and_Resource_Partitioning__IRP_.tex <==
\subsection{Isolation and Resource Partitioning (IRP):} Isolation and resource partitioning techniques play a pivotal role in mitigating memory side-channel attacks by ensuring strict separation of shared resources and minimizing cross-process interference. These strategies aim to provide robust defenses against adversarial activities in multi-tenant and shared environments.

One prominent strategy involves cache isolation and partitioning. Low-complexity cache designs employ innovative structures to prevent monopolization by adversarial processes. By limiting an attacker’s ability to dominate cache resources, these designs effectively reduce contention in shared environments\cite{domnitser2012non}. Dynamic partitioning of last-level caches (LLCs) ensures minimal interference between processes by using cache allocation technology. \textit{fiore et al.} dynamically allocates cache resources to balance system performance and enhance isolation. On-demand and scalable cache isolation mechanisms dynamically isolate cache regions, adapting to varying workloads to improve flexibility. Additionally, reconfigured cache layouts mitigate predictable access patterns, reducing an attacker’s ability to infer sensitive data while enhancing system adaptability\cite{song2022remapped}. Set-based partitioning techniques further reduce contention by allocating specific cache sets to individual applications or threads, enhancing overall system security\cite{dessouky2021chunked}.

Scheduler-based techniques also play a significant role in resource partitioning. CPU core pinning assigns dedicated cores to specific processes to isolate sensitive tasks from potential adversaries. By preventing cross-thread data leakage, it enhances security in shared environments \cite{sprabery2018scheduling}. Task scheduling algorithms manage process execution to avoid simultaneous access to shared resources by adversaries which, ensures isolation and enhances system resilience against side-channel threats \cite{varadarajan2014scheduler}. Scheduling algorithms integrated with cache allocation policies isolate critical operations by assigning specific resources to secure tasks. This dual approach balances security with system throughput, reducing adversarial influence \cite{sprabery2018scheduling}.

Memory timing defenses form another pillar of resource partitioning. Memory access isolation prevents observable patterns that could reveal sensitive data, thereby fortifying enclave defenses against practical side-channel attacks \cite{oleksenko2018varys}. Memory access obfuscation randomizes access patterns to disrupt an attacker’s ability to make timing-based inferences which, significantly enhances the security of sensitive computations\cite{deutsch2022dagguise}. Memory encryption techniques protect sensitive data by encrypting virtual machine (VM) memory to prevent unauthorized access. This method mitigates physical attacks and preserves sensitive computation integrity, ensuring confidentiality even in compromised environments\cite{geng2024new}.

These isolation and resource partitioning strategies collectively provide robust defenses against memory side-channel attacks. They address vulnerabilities across shared and multi-tenant environments by integrating separation mechanisms at the cache, CPU, and memory levels, ensuring comprehensive protection. They form a critical component of comprehensive security frameworks, mitigating risks while preserving performance in modern computing systems.

==> Sections/Miscelleneous/Software_Level_Mitigations__SLM_.tex <==
\subsection{Software Level Mitigations (SLM):} Software-level mitigations play a pivotal role in defending against memory side-channel attacks by addressing vulnerabilities at the operating system, library, and application levels. Unlike hardware-based defenses, these techniques are versatile, cost-effective, and can often be deployed on existing systems without requiring physical upgrades. By implementing strategies that modify memory access patterns, obfuscate execution, and enforce randomness, software-level mitigations provide essential protection against evolving attack methodologies.
One prominent approach involves retrofitting existing systems to reduce side-channel leakage. Techniques to minimize cache interference and mitigate leakage in multi-tenant environments\cite{zhou2016software}. These foundational strategies seamlessly integrate with techniques targeting speculative execution and obfuscation to create a robust defense framework. Methods modifying operating systems to mitigate cache-based side channels \cite{zhang2013duppel} modifies commodity operating systems to mitigate cache-based side channels in cloud environments by introducing noise into memory access patterns, effectively masking sensitive operations. Similarly, Exitless OS services for SGX enclaves enables exitless OS services for SGX enclaves, reducing the frequency of context switches and, thereby, minimizing the attack surface exposed to adversaries\cite{orenbach2017eleos}. Dynamic memory randomization during execution dynamically randomizes software memory layouts during execution, thwarting adversaries attempting to exploit predictable memory mappings\cite{chen2016remix}.
Another critical strategy involves implementing techniques to defend against speculative execution and cache timing attacks. [\textit{elatali et al.} transparently mitigate Spectre-like attacks by allowing speculative memory operations to be revoked before they leak information. Randomized cache line replacement policies  introduces randomness in cache line replacement policies to prevent timing-based attacks by making access patterns less predictable\cite{wang2020mitigating}. Techniques restricting privileged code observation \cite{dong2018shielding} further strengthens protections by restricting privileged code’s ability to observe sensitive software states, effectively neutralizing high-privilege side-channel attacks. Evaluations of countermeasure effectiveness systematically evaluates the effectiveness of various countermeasures, providing critical insights for optimizing defenses against cache-based leakage\cite{doychev2017rigorous}. Page table randomization approaches employs page table randomization to proactively defend SGX enclaves against page-table-based side channels, either detecting or preventing attacks before sensitive data is leaked\cite{strackx2017heisenberg}.
Obfuscation and software diversity techniques also play a vital role in disrupting side-channel attacks. Obfuscation engines for Intel SGX \cite{ahmad2019obfuscuro} operates as a commodity obfuscation engine for Intel SGX, encrypting and diversifying application code to make it resistant to microarchitectural attacks. Dynamic software diversity techniques builds upon this by dynamically altering software execution paths and memory layouts, creating significant uncertainty for attackers\cite{crane2015thwarting} while automated program transformation techniques \cite{li2020dlfix} automates the process of modifying application code to eliminate timing-based side channels, ensuring a systematic and scalable approach to defending against these attacks. Prefetching noise mechanisms introduced by \textit{li et al.}, prefetching noise as a defense mechanism, using intelligent prefetching to obscure real access patterns and enhance security while maintaining performance\cite{li2024p}.
Software-level mitigations also address memory-resident sensitive data, ensuring its security even in shared or vulnerable environments. Memory-resident sensitive data protection techniques protects sensitive data by encrypting or isolating it during processing, rendering it inaccessible to adversaries probing for residual traces\cite{palit2019mitigating}. \textit{brasser et al.} hardens SGX enclaves against cache attacks through data location randomization, preventing attackers from leveraging deterministic memory layouts to infer sensitive information\cite{brasser2017dr}. System-level protections locking critical cache lines \cite{kim2012stealthmem} introduces system-level protections that prevent sensitive data from being evicted from caches by locking critical cache lines, reducing opportunities for leakage. Page table isolation mechanisms enhances security by isolating page tables to block unauthorized access, particularly addressing Meltdown-style vulnerabilities\cite{tan2023ptstore}.
Despite challenges like performance overhead and implementation complexity, software-level mitigations are adaptable and indispensable. As memory side-channel attacks evolve, these defenses must continuously innovate to address emerging vulnerabilities and remain effective. They complement hardware solutions, forming a layered defense strategy to counter evolving memory side-channel attacks.


==> Tables/Comparisontable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\caption{Comparison of Different Memory-based Side-channel Attacks}
\label{tab:comparison-table}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|cccc|c|c|c|cc|}
\hline
\multirow{2}{*}{\textbf{Literature(Year)}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Type}\end{tabular}} &
  \multirow{2}{*}{\textbf{Target}} &
  \multirow{2}{*}{\textbf{Methodology}} &
  \multicolumn{4}{c|}{\textbf{Platform}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Vulnerable}\\\textbf{Component}\end{tabular}} &
  \multirow{2}{*}{\textbf{Impact}} &
  \multirow{2}{*}{\textbf{Complexity}} &
  \multicolumn{2}{c|}{\textbf{Mitigations}} \\ \cline{5-8} \cline{12-13} 
 &
   &
   &
   &
  \multicolumn{1}{c|}{\textbf{Intel}} &
  \multicolumn{1}{c|}{\textbf{AMD}} &
  \multicolumn{1}{c|}{\textbf{ARM}} &
  \textbf{Cross} &
   &
   &
   &
  \multicolumn{1}{c|}{\textbf{SW}} &
  \textbf{HW} \\ \hline\hline
  Dall et al. (2018) &
  CTA &
  SGX EPID &
  Prime+Probe &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L1 Data Cache &
  Key Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  van Schaik et al. (2021)) &
  CTA &
  SGX EPID &
  Prime+Probe &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm & Cache &
  Key Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Ragab et al. (2021) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}SGX Enclave Random\\ Number Generators \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Transient Execution\\Staging Buffer Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Shared Staging Buffer\\ Microcode \end{tabular} &
  Key Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Zhang et al. (2012) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Co-Resident VMs\\Cryptographic Keys \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prime+Probe\\Access-Driven \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L1 Instruction Cache &
  Key Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Pessl et al. (2016) &
  MBA &
  \begin{tabular}[c]{@{}c@{}}DRAM Modules \\Cross-CPU Memory \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Rowhammer Exploits \\DRAM Address Mapping \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \cm &
  \begin{tabular}[c]{@{}c@{}} DRAM Rows \& Buffers \end{tabular} &
  Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  van der Veen et al. (2016) &
  MBA &
  \begin{tabular}[c]{@{}c@{}}Mobile DRAM \\ARM Processors \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Deterministic Rowhammer \\Flip Feng Shui \end{tabular} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\cm} &
  \xm &
  DRAM Rows and Allocators &
  Data Corruption &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Canella et al. (2019) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Store Buffer\\Kernel Writes \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Store-to-Leak Write\\ Transient Forwarding (WTF) \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Store Buffer \\TLB \end{tabular} &
  Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Kim et al. (2014) &
  MBA &
  DRAM Cells &
  Rowhammer Disturbance Error &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \cm &
  DRAM Wordlines &
  Data Corruption &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Yarom et al. (2014) (2018) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Shared Memory Pages \\L3 Cache \end{tabular} &
  Flush+Reload &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L3 Cache &
  Key Leakage &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Gruss et al. (2016) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Shared Memory \\Cache Timing \end{tabular} &
  Flush+Flush &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L3 Cache &
  Stealthy Data Leakage &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Weisse et al. (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Virtual Memory \\L1 Cache \end{tabular} &
  L1 Terminal Fault (L1TF) &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L1 Data Cache &
  Sensitive Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Van Bulck et al. (2018) &
  TSEA &
  Intel SGX Enclaves &
  Speculative Execution Bug &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L1 Cache &
  Key Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Lee et al. (2017) &
  ETA &
  \begin{tabular}[c]{@{}c@{}}SGX Branch History \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Branch Shadowing \\APIC Timer Manipulation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Branch Target Buffer (BTB) &
  Cryptographic Key Leakage &
  High &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  Gruss et al. (2016) &
  PTA &
  \begin{tabular}[c]{@{}c@{}}Kernel Address \\Layout \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prefetch Instruction \\Double Page Fault \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Page Table \\TLB \end{tabular} &
  KASLR Bypass
  &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Evtyushkin et al. (2016) &
  TSEA &
  User and Kernel ASLR &
  \begin{tabular}[c]{@{}c@{}}BTB Collisions \\Branch Predictor Exploitation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Branch Target Buffer (BTB) &
  ASLR Bypass &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Liu et al. (2015) &
  CTA &
  Last-Level Cache (LLC) &
  \begin{tabular}[c]{@{}c@{}}Prime+Probe \\Temporal Access Patterns \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Last Lvele Cache \\Cache Slices \end{tabular} &
  Cryptographic Key Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Stecklina \& Prescher (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}FPU \& \\SIMD Registers \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Speculative Execution \\Cache Side Effects \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  FPU Registers &
 \begin{tabular}[c]{@{}c@{}}Data Leakage \\Across Contexts \end{tabular} &
  Moderate &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  Van Bulck et al. (2020) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}SGX Enclaves \\Kernel Isolation \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Load Value Injection \\Gadgets \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Microarchitectural Buffers &
  Data Leakage &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Trippel et al. (2018) &
  CTA &
  Cache Coherence Protocols &
  Prime+Probe Variants &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Last-Level Cache (LLC) &
  Cache Coherence &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Moghimi et al. (2019) &
  MBA &
  \begin{tabular}[c]{@{}c@{}}Shared Buffers \\Memory Bus \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Write Combining \\Fill Buffer Exploit \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Fill Buffer \\WC Buffer \end{tabular} &
  Precise Data Leakage &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Schwarz et al. (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Remote Systems \\via Network \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Remote Spectre Variant 1, \\Thrash+Reload, \\AVX Covert Channel \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Cache System \\Spectre Gadgets Mechanism \end{tabular} &
  Data Leakage Over Network &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Gruss et al. (2019) &
  PTA &
  \begin{tabular}[c]{@{}c@{}}Page Cache in \\Operating Systems \end{tabular} &
  Page Cache State Analysis &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  Page Cache &
 Data Leakage &
  Moderate &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Murdock et al. (2020) &
  FIA &
  Intel SGX Enclaves &
  \begin{tabular}[c]{@{}c@{}}Voltage Undervolting \\SGX Fault Induction \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Voltage Regulation &
  Data Integrity Breach &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Hund et al. (2013) &
  PTA &
  Kernel Space ASLR &
  \begin{tabular}[c]{@{}c@{}}Kernel Memory \\Timing Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Cache Hierarchy &
  Kernel ASLR Bypass &
  Moderate &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Gruss et al. (2016) &
  PTA &
  \begin{tabular}[c]{@{}c@{}}Kernel ASLR Physical\\Memory Access \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prefetch Instruction \\Translation-Level Oracle \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  \begin{tabular}[c]{@{}c@{}} Prefetch Mechanism \\Cache Hierarchy Mechanism \end{tabular} &
 \begin{tabular}[c]{@{}c@{}}KSLR Compromise\end{tabular} &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Schwarzl et al. (2023) &
  ETA &
  \begin{tabular}[c]{@{}c@{}}Memory Compression\\ Algorithms \\Remote Interfaces \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Timing Analysis \\Memory Compression Timing \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  Compression Algorithms &
  Data Leakage &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Disselkoen et al. (2017) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}L3 Cache, \\Shared Memory \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Intel TSX Exploitation, \\Prime+Abort  \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} L3 Cache \\TSX Implementation \end{tabular} &
 \begin{tabular}[c]{@{}c@{}} Precise Cache \\Behavior Monitoring \end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Shusterman et al. (2021) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Web Browsers \\Resource Access \end{tabular} &
  Cache Contention Analysis &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  Browser Cache Mechanisms &
  Resource Leakage &
  Moderate &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Kemerlis et al. (2014) &
  PTA &
  \begin{tabular}[c]{@{}c@{}}Linux Kernel Physical\\ Memory Mappings \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Direct Mapped Memory \\Return-to-User Variant \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  \begin{tabular}[c]{@{}c@{}}Memory Management\\ Subsystem\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Kernel Address\\ Space Leakage\end{tabular} &
  Moderate &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  Maisuradze et al. (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Return Address Prediction\\ Units JIT Environments \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}RSB Manipulation \\Speculative Code Execution \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Branch Prediction Units &
 \begin{tabular}[c]{@{}c@{}} Data Leakage Across \\Speculative Paths \end{tabular} &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Mutlu \& Kim et al. (2019) &
  MBA &
  \begin{tabular}[c]{@{}c@{}}Adjacent DRAM Rows \\Kernel Privileges \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}DRAM Disturbance \\Row Activation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  DRAM Row Architecture &
  System Security Compromise &
  Moderate &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  van Schaik et al. (2019) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Intel CPUs \\Security Boundaries \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Line Fill Buffer \\Speculative Data Leaks \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Microarchitectural Buffers &
 \begin{tabular}[c]{@{}c@{}} Arbitrary Data Leaks \\Across Boundaries \end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Chen et al. (2019) &
  TSEA &
  Intel SGX Enclaves &
  Branch Target Injection &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}}Branch Prediction Units \\Cache Hierarchy\end{tabular} &
 \begin{tabular}[c]{@{}c@{}} Confidentiality Breach of \\SGX Enclaves \end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Bhattacharyya et al. (2019) &
  TSEA &
  Multi-Threaded Processors &
  \begin{tabular}[c]{@{}c@{}}Port Contention Analysis \\Speculative Gadget Execution \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Execution Ports \\Speculative Control Flow \end{tabular} &
  Speculative Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Brasser et al. (2017) &
  CTA &
  Intel SGX Enclaves &
  \begin{tabular}[c]{@{}c@{}}Cache Monitoring \\Performance Counter\\ Exploitation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} L1 Cache \\Cache Architecture \end{tabular} &
  Cryptographic Data Leakage &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Koruyeh et al. (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Intel CPUs \\SGX Enclaves \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Return Stack Buffer \\Speculative Gadget \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Return Stack Buffer &
 \begin{tabular}[c]{@{}c@{}} Data Leakage via \\Speculative Paths \end{tabular} &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Gras et al. (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Translation Lookaside\\ Buffers, Shared Resources \end{tabular} &
  ML Based Temporal Analysis &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}}TLB Sets \& \\Mapping Function\end{tabular} &
  Data Leakage via TLBs &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Oren et al. (2015) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Web Browsers \\Shared L3 Cache \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prime+Probe \\Covert Channel Monitoring \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L3 Cache &
  Private Browsing Leakage &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Van Bulck et al. (2017) &
  PTA &
  Intel SGX Enclaves &
  \begin{tabular}[c]{@{}c@{}}Page Table\\ Attribute Manipulation\end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Page Table Attributes &
  Data Leakage via Page Tables &
  High &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  Yan et al. (2020) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}DNN Architectures on \\Shared CPUs \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prime+Probe \\Flush+Reload DNN\\ Hyper Parameter Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Shared Cache Resources &
  Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Shinde et al. (2016) &
  PTA &
  \begin{tabular}[c]{@{}c@{}}Cryptographic Routines \\(AES, EdDSA), Intel SGX \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Page Fault Channe \\Pigeonhole Attacks \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}}Page Fault Patterns \\OS Memory Management \end{tabular} &
  Leakage of Secret Bits &
  High &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  Kwong et al. (2020) &
  MBA &
  \begin{tabular}[c]{@{}c@{}}ECC Memory \\Shared DRAM Rows \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Rowhammer-Induced Read\\ Channel ECC Exploitation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Rowhammer Effects \\ECC Correction Timing \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Confidentiality Breach\\ of Memory\end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Schwarz et al. (2017) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Co-Located Enclaves \\RSA Implementations \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prime+Probe \\DRAM and Cache Exploitation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Shared Cache Resources &
  \begin{tabular}[c]{@{}c@{}}Data Exfiltration from\\ SGX Enclaves\end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Xu et al. (2015) &
  PTA &
  \begin{tabular}[c]{@{}c@{}}Protected Applications \\on Shielding Systems \end{tabular} &
  Page Table Manipulation &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Page Fault Management &
  Data Leakage via Page Faults &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Moghimi et al. (2019) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}SGX Enclaves \\Constant-Time AES \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}False Dependency \\4K Aliasing \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Cache Hierarchy\\ Memory R/W Dependencies \end{tabular} &
  Confidentiality Breach &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Tang et al. (2017) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}ARM TrustZone \\AES Keys \end{tabular} &
  (DVFS) Manipulation &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\cm} &
  \xm &
  Energy Management Interfaces &
 \begin{tabular}[c]{@{}c@{}} Fault Induction \\Cryptographic Key Leakage \end{tabular} &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Aciicmez et al. (2007) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}RSA Cryptosystems, \\Instruction Paths \end{tabular} &
  Instruction Cache Analysis &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Instruction Cache &
  Data Leakage via I-cache &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Moghimi et al. (2020) &
  PTA &
  Intel SGX Enclaves &
  \begin{tabular}[c]{@{}c@{}}Controlled-Channel Attacks \\Instruction-Level Counting \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}}Paging and Instruction-Level\\ Operations\end{tabular} &
  Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Barresi et al. (2016) &
  PTA &
  \begin{tabular}[c]{@{}c@{}}Virtual Machines \\Cloud Infrastructures \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Memory Deduplication \\Timing Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}}Memory Deduplication\\ Mechanism\end{tabular} &
 \begin{tabular}[c]{@{}c@{}} Breaking ASLR in \\Multi-Tenant Environments \end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Irazoqui et al. (2015) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Last Level Cache \\AES Implementations \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prime+Probe \\Shared Cache Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Shared Cache \\Huge Pages \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Data Confidentiality\\ Compromise\end{tabular} &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Zhang et al. (2012) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Symmetric Multiprocessing \\Xen Virtual Machines\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Access-Driven Cache Analysis \\ElGamal Key Extraction \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L1 Data Cache &
 \begin{tabular}[c]{@{}c@{}} Private Key Leakage \\in Virtualized Environments \end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Gras et al. (2017) &
  PTA &
  Memory Management Unit &
  \begin{tabular}[c]{@{}c@{}}Evict+Time \\Page Table Walk Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \xm &
  Shared Cache, MMU &
 \begin{tabular}[c]{@{}c@{}} Breaking ASLR in \\Sandboxed Environments\end{tabular} &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  





\end{tabular}
}
\end{table*}




\begin{table*}[!ht]
\ContinuedFloat 
\caption{Comparison of Different Memory-based Side-channel Attacks}
\label{tab:comparison-table}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|cccc|c|c|c|cc|}
\hline
\multirow{2}{*}{\textbf{Literature(Year)}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Attack}\\ \textbf{Category}\end{tabular}} &
  \multirow{2}{*}{\textbf{Target}} &
  \multirow{2}{*}{\textbf{Methodology}} &
  \multicolumn{4}{c|}{\textbf{Platform}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Vulnerable}\\\textbf{Component}\end{tabular}} &
  \multirow{2}{*}{\textbf{Impact}} &
  \multirow{2}{*}{\textbf{Complexity}} &
  \multicolumn{2}{c|}{\textbf{Mitigations}} \\ \cline{5-8} \cline{12-13} 
 &
   &
   &
   &
  \multicolumn{1}{c|}{\textbf{Intel}} &
  \multicolumn{1}{c|}{\textbf{AMD}} &
  \multicolumn{1}{c|}{\textbf{ARM}} &
  \textbf{Cross} &
   &
   &
   &
  \multicolumn{1}{c|}{\textbf{SW}} &
  \textbf{HW} \\ \hline\hline


Evtyushkin et al. (2018) &
  ETA &
  \begin{tabular}[c]{@{}c@{}}Directional Branch\\ Predictors Intel SGX \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Directional Predictor\\ Manipulation Collisions in\\ Branch Prediction Tables \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Branch Prediction Unit &
  Data Exfiltration &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Gullasch et al. (2011) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}AES Implementations \\(OpenSSL)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Access-Driven Cache Timing \\Neural Network Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Shared Cache, Task Scheduler &
  Cryptographic Key Leakage &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Gruss et al. (2015) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Inclusive Last-Level Caches \\Cryptographic Libraries \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Flush+Reload \\Automated Cache Profiling \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Last-Level Cache &
  Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Yarom et al. (2017) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Scatter-Gather RSA\\ Implementations (OpenSSL)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Cache-Bank Conflict \\False Dependency \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}}Cache-Bank Structures \\Scatter-Gather Mechanism\end{tabular} &
 \begin{tabular}[c]{@{}c@{}} Cryptographic Key Leakage \end{tabular} &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Lipp et al. (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Kernel Memory \\Physical Memory\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Out-of-Order Execution \\Microarchitectural Covert Channels \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \xm &
  Out-of-Order Execution &
  Memory Isolation Violations &
  Moderate &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  Frigo et al. (2020) &
  MBA &
  \begin{tabular}[c]{@{}c@{}}Quoting Enclave\\EPID protocol \end{tabular} &
  DDR4, LPDDR4(X) DRAM &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \xm &
  RowHammer Mitigation (TRR) &
 \begin{tabular}[c]{@{}c@{}}Memory Corruption \\Data Integrity Violations\end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Islam et al. (2019) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Memory Subsystem \\Cache Timing \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Dependency Resolution \\RowHammer Enhancement \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  Speculative Load Operations &
  Efficient RowHammer Triggering &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Wang et al. (2017) &
  PTA &
  Intel SGX Enclaves &
  \begin{tabular}[c]{@{}c@{}}Page-Fault Analysis \\Address Translation Leaks \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Page Tables \\Translation lookaside Buffer \end{tabular} &
 \begin{tabular}[c]{@{}c@{}} Data Leakage in \\SGX Applications \end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Kocher et al. (2018) &
  TSEA &
  \begin{tabular}[c]{@{}c@{}}Kernel Memory\\User Processes \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Speculative Execution \\Microarchitectural Covert Channels \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  Speculative Execution &
  System Security Breach &
  High &
  \multicolumn{1}{c|}{\cm} &
  \cm \\ \hline

  Schwarz et al. (2017) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Browsers \\Virtual Machines \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}High-Resolution \\Timer Exploitation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \cm &
  JavaScript Timer API &
 \begin{tabular}[c]{@{}c@{}} Data Leakage \\from Browsers \end{tabular} &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Allan et al. (2016) &
  RCA &
  \begin{tabular}[c]{@{}c@{}}Shared Caches \\OpenSSL ECDSA \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Cache Eviction \\Performance Degradation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} Shared Cache, \\Resource Scheduling \end{tabular} &
   Data Leakage &
  High &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline

  Bhattacharya et al. (2016) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Cryptographic Keys \\in DRAM \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Timing Analysis \\Rowhammer Exploitation \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  \begin{tabular}[c]{@{}c@{}} DRAM Rows \\Row Buffers \end{tabular} &
  Cryptographic Vulnerabilities &
  High &
  \multicolumn{1}{c|}{\cm} &
  \xm \\ \hline

  Lipp et al. (2016) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}ARM CPUs \\Mobile Devices\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Prime+Probe \\Evict+Reload \\Flush+Reload \end{tabular} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\cm} &
  \xm &
  Last-Level Caches &
  Mobile Device &
  High &
  \multicolumn{1}{c|}{\xm} &
  \cm \\ \hline

  Percival et al. (2005) &
  CTA &
  \begin{tabular}[c]{@{}c@{}}Shared Caches in \\Multithread Environments \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Shared Cache \\Covert Channels \end{tabular} &
  \multicolumn{1}{c|}{\cm} &
  \multicolumn{1}{c|}{\xm} &
  \multicolumn{1}{c|}{\xm} &
  \xm &
  L1, L2 Caches &
 \begin{tabular}[c]{@{}c@{}} Data Leakage in Shared Caches \end{tabular} &
  Moderate &
  \multicolumn{1}{c|}{\xm} &
  \xm \\ \hline




\end{tabular}
}
\end{table*}

==> ref.tex <==
1=> roy2022survey

==> ref_backup.tex <==
%%1
@article{roy2022survey,
  title={Survey and taxonomy of adversarial reconnaissance techniques},
  author={Roy, Shanto and Sharmin, Nazia and Acosta, Jaime C and Kiekintveld, Christopher and Laszka, Aron},
  journal={ACM Computing Surveys},
  volume={55},
  number={6},
  pages={1--38},
  year={2022},
  publisher={ACM New York, NY}
}

@periodical{bush:1945:awmt,
    title = {As We May Think}, 
    journal = {The Atlantic Monthly}, 
    organization = {The Atlantic},
    volume = {176}, 
    number = {1}, 
    pages = {101--108}, 
    year = {1945}, 
    url = {http://www.theatlantic.com/magazine/archive/1945/07/as-we-may-think/303881/}, 
    lastaccessed = {August 7, 2023}
}




@article{lipp2020meltdown,
  title={Meltdown: Reading kernel memory from user space},
  author={Lipp, Moritz and Schwarz, Michael and Gruss, Daniel and Prescher, Thomas and Haas, Werner and Horn, Jann and Mangard, Stefan and Kocher, Paul and Genkin, Daniel and Yarom, Yuval and others},
  journal={Communications of the ACM},
  volume={63},
  number={6},
  pages={46--56},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{kim2014flipping,
  title={Flipping bits in memory without accessing them: An experimental study of DRAM disturbance errors},
  author={Kim, Yoongu and Daly, Ross and Kim, Jeremie and Fallin, Chris and Lee, Ji Hye and Lee, Donghyuk and Wilkerson, Chris and Lai, Konrad and Mutlu, Onur},
  journal={ACM SIGARCH Computer Architecture News},
  volume={42},
  number={3},
  pages={361--372},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@inproceedings{van2017telling,
  title={Telling your secrets without page faults: Stealthy page Table-Based attacks on enclaved execution},
  author={Van Bulck, Jo and Weichbrodt, Nico and Kapitza, R{\"u}diger and Piessens, Frank and Strackx, Raoul},
  booktitle={26th USENIX Security Symposium (USENIX Security 17)},
  pages={1041--1056},
  year={2017}
}

@inproceedings{chen2019sgxpectre,
  title={Sgxpectre: Stealing intel secrets from sgx enclaves via speculative execution},
  author={Chen, Guoxing and Chen, Sanchuan and Xiao, Yuan and Zhang, Yinqian and Lin, Zhiqiang and Lai, Ten H},
  booktitle={2019 IEEE European Symposium on Security and Privacy (EuroS\&P)},
  pages={142--157},
  year={2019},
  organization={IEEE}
}

@inproceedings{zhou2016software,
  title={A software approach to defeating side channels in last-level caches},
  author={Zhou, Ziqiao and Reiter, Michael K and Zhang, Yinqian},
  booktitle={Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
  pages={871--882},
  year={2016}
}

@inproceedings{gruss2015cache,
  title={Cache template attacks: Automating attacks on inclusive Last-Level caches},
  author={Gruss, Daniel and Spreitzer, Raphael and Mangard, Stefan},
  booktitle={24th USENIX Security Symposium (USENIX Security 15)},
  pages={897--912},
  year={2015}
}

@inproceedings{koruyeh2018spectre,
  title={Spectre returns! speculation attacks using the return stack buffer},
  author={Koruyeh, Esmaeil Mohammadian and Khasawneh, Khaled N and Song, Chengyu and Abu-Ghazaleh, Nael},
  booktitle={12th USENIX Workshop on Offensive Technologies (WOOT 18)},
  year={2018}
}

@article{chowdhuryy2021leaking,
  title={Leaking secrets through modern branch predictors in the speculative world},
  author={Chowdhuryy, Md Hafizul Islam and Yao, Fan},
  journal={IEEE Transactions on Computers},
  volume={71},
  number={9},
  pages={2059--2072},
  year={2021},
  publisher={IEEE}
}

@article{mcilroy2019spectre,
  title={Spectre is here to stay: An analysis of side-channels and speculative execution},
  author={Mcilroy, Ross and Sevcik, Jaroslav and Tebbi, Tobias and Titzer, Ben L and Verwaest, Toon},
  journal={arXiv preprint arXiv:1902.05178},
  year={2019}
}

@article{evtyushkin2018branchscope,
  title={Branchscope: A new side-channel attack on directional branch predictor},
  author={Evtyushkin, Dmitry and Riley, Ryan and Abu-Ghazaleh, Nael CSE and ECE and Ponomarev, Dmitry},
  journal={ACM SIGPLAN Notices},
  volume={53},
  number={2},
  pages={693--707},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@inproceedings{gruss2016flush+,
  title={Flush+ Flush: a fast and stealthy cache attack},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Wagner, Klaus and Mangard, Stefan},
  booktitle={Detection of Intrusions and Malware, and Vulnerability Assessment: 13th International Conference, DIMVA 2016, San Sebasti{\'a}n, Spain, July 7-8, 2016, Proceedings 13},
  pages={279--299},
  year={2016},
  organization={Springer}
}

@inproceedings{yarom2014flush+,
  title={FLUSH+ RELOAD: A high resolution, low noise, l3 cache Side-Channel attack},
  author={Yarom, Yuval and Falkner, Katrina},
  booktitle={23rd USENIX security symposium (USENIX security 14)},
  pages={719--732},
  year={2014}
}

@inproceedings{gruss2016prefetch,
  title={Prefetch side-channel attacks: Bypassing SMAP and kernel ASLR},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Fogh, Anders and Lipp, Moritz and Mangard, Stefan},
  booktitle={Proceedings of the 2016 ACM SIGSAC conference on computer and communications security},
  pages={368--379},
  year={2016}
}

@article{kiriansky2018speculative,
  title={Speculative buffer overflows: Attacks and defenses},
  author={Kiriansky, Vladimir and Waldspurger, Carl},
  journal={arXiv preprint arXiv:1807.03757},
  year={2018}
}

@inproceedings{canella2019fallout,
  title={Fallout: Leaking data on meltdown-resistant cpus},
  author={Canella, Claudio and Genkin, Daniel and Giner, Lukas and Gruss, Daniel and Lipp, Moritz and Minkin, Marina and Moghimi, Daniel and Piessens, Frank and Schwarz, Michael and Sunar, Berk and others},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={769--784},
  year={2019}
}

@inproceedings{van2019ridl,
  title={RIDL: Rogue in-flight data load},
  author={Van Schaik, Stephan and Milburn, Alyssa and {\"O}sterlund, Sebastian and Frigo, Pietro and Maisuradze, Giorgi and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={88--105},
  year={2019},
  organization={IEEE}
}

@inproceedings{schwarz2019zombieload,
  title={ZombieLoad: Cross-privilege-boundary data sampling},
  author={Schwarz, Michael and Lipp, Moritz and Moghimi, Daniel and Van Bulck, Jo and Stecklina, Julian and Prescher, Thomas and Gruss, Daniel},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={753--768},
  year={2019}
}

@inproceedings{moghimi2020copycat,
  title={CopyCat: Controlled Instruction-Level attacks on enclaves},
  author={Moghimi, Daniel and Van Bulck, Jo and Heninger, Nadia and Piessens, Frank and Sunar, Berk},
  booktitle={29th USENIX security symposium (USENIX security 20)},
  pages={469--486},
  year={2020}
}

@inproceedings{van2021cacheout,
  title={CacheOut: Leaking data on Intel CPUs via cache evictions},
  author={Van Schaik, Stephan and Minkin, Marina and Kwong, Andrew and Genkin, Daniel and Yarom, Yuval},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={339--354},
  year={2021},
  organization={IEEE}
}

@inproceedings{ragab2021crosstalk,
  title={Crosstalk: Speculative data leaks across cores are real},
  author={Ragab, Hany and Milburn, Alyssa and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={1852--1867},
  year={2021},
  organization={IEEE}
}

@inproceedings{younis2015new,
  title={A new prime and probe cache side-channel attack for cloud computing},
  author={Younis, Younis A and Kifayat, Kashif and Shi, Qi and Askwith, Bob},
  booktitle={2015 IEEE International Conference on Computer and Information Technology; Ubiquitous Computing and Communications; Dependable, Autonomic and Secure Computing; Pervasive Intelligence and Computing},
  pages={1718--1724},
  year={2015},
  organization={IEEE}
}

@article{mutlu2019rowhammer,
  title={Rowhammer: A retrospective},
  author={Mutlu, Onur and Kim, Jeremie S},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={8},
  pages={1555--1571},
  year={2019},
  publisher={IEEE}
}

@inproceedings{van2016drammer,
  title={Drammer: Deterministic rowhammer attacks on mobile platforms},
  author={Van Der Veen, Victor and Fratantonio, Yanick and Lindorfer, Martina and Gruss, Daniel and Maurice, Cl{\'e}mentine and Vigna, Giovanni and Bos, Herbert and Razavi, Kaveh and Giuffrida, Cristiano},
  booktitle={Proceedings of the 2016 ACM SIGSAC conference on computer and communications security},
  pages={1675--1689},
  year={2016}
}

@inproceedings{zhang2012cross,
  title={Cross-VM side channels and their use to extract private keys},
  author={Zhang, Yinqian and Juels, Ari and Reiter, Michael K and Ristenpart, Thomas},
  booktitle={Proceedings of the 2012 ACM conference on Computer and communications security},
  pages={305--316},
  year={2012}
}

@inproceedings{lee2017inferring,
  title={Inferring fine-grained control flow inside $\{$SGX$\}$ enclaves with branch shadowing},
  author={Lee, Sangho and Shih, Ming-Wei and Gera, Prasun and Kim, Taesoo and Kim, Hyesoon and Peinado, Marcus},
  booktitle={26th USENIX Security Symposium (USENIX Security 17)},
  pages={557--574},
  year={2017}
}

@article{evtyushkin2018branchscope,
  title={Branchscope: A new side-channel attack on directional branch predictor},
  author={Evtyushkin, Dmitry and Riley, Ryan and Abu-Ghazaleh, Nael CSE and ECE and Ponomarev, Dmitry},
  journal={ACM SIGPLAN Notices},
  volume={53},
  number={2},
  pages={693--707},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@inproceedings{xu2015controlled,
  title={Controlled-channel attacks: Deterministic side channels for untrusted operating systems},
  author={Xu, Yuanzhong and Cui, Weidong and Peinado, Marcus},
  booktitle={2015 IEEE Symposium on Security and Privacy},
  pages={640--656},
  year={2015},
  organization={IEEE}
}

@inproceedings{kemerlis2014ret2dir,
  title={ret2dir: Rethinking kernel isolation},
  author={Kemerlis, Vasileios P and Polychronakis, Michalis and Keromytis, Angelos D},
  booktitle={23rd USENIX Security Symposium (USENIX Security 14)},
  pages={957--972},
  year={2014}
}

@inproceedings{gras2018translation,
  title={Translation leak-aside buffer: Defeating cache side-channel protections with $\{$TLB$\}$ attacks},
  author={Gras, Ben and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={955--972},
  year={2018}
}
@inproceedings{yan2020cache,
  title={Cache telepathy: Leveraging shared resource attacks to learn $\{$DNN$\}$ architectures},
  author={Yan, Mengjia and Fletcher, Christopher W and Torrellas, Josep},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={2003--2020},
  year={2020}
}

@article{weisse2018foreshadow,
  title={Foreshadow-NG: Breaking the virtual memory abstraction with transient out-of-order execution},
  author={Weisse, Ofir and Van Bulck, Jo and Minkin, Marina and Genkin, Daniel and Kasikci, Baris and Piessens, Frank and Silberstein, Mark and Strackx, Raoul and Wenisch, Thomas F and Yarom, Yuval},
  year={2018}
}

@inproceedings{van2018foreshadow,
  title={Foreshadow: Extracting the keys to the intel $\{$SGX$\}$ kingdom with transient $\{$Out-of-Order$\}$ execution},
  author={Van Bulck, Jo and Minkin, Marina and Weisse, Ofir and Genkin, Daniel and Kasikci, Baris and Piessens, Frank and Silberstein, Mark and Wenisch, Thomas F and Yarom, Yuval and Strackx, Raoul},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={991--1008},
  year={2018}
}

@inproceedings{murdock2020plundervolt,
  title={Plundervolt: Software-based fault injection attacks against Intel SGX},
  author={Murdock, Kit and Oswald, David and Garcia, Flavio D and Van Bulck, Jo and Gruss, Daniel and Piessens, Frank},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={1466--1482},
  year={2020},
  organization={IEEE}
}

@inproceedings{cui2021smashex,
  title={Smashex: Smashing sgx enclaves using exceptions},
  author={Cui, Jinhua and Yu, Jason Zhijingcheng and Shinde, Shweta and Saxena, Prateek and Cai, Zhiping},
  booktitle={Proceedings of the 2021 ACM SIGSAC conference on computer and communications security},
  pages={779--793},
  year={2021}
}
@article{sridhara2024sigy,
  title={SIGY: Breaking Intel SGX Enclaves with Malicious Exceptions \& Signals},
  author={Sridhara, Supraja and Bertschi, Andrin and Schl{\"u}ter, Benedict and Shinde, Shweta},
  journal={arXiv preprint arXiv:2404.13998},
  year={2024}
}

@inproceedings{cloosters2020teerex,
  title={$\{$TeeRex$\}$: Discovery and exploitation of memory corruption vulnerabilities in $\{$SGX$\}$ enclaves},
  author={Cloosters, Tobias and Rodler, Michael and Davi, Lucas},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={841--858},
  year={2020}
}

@inproceedings{kocher1996timing,
  title={Timing attacks on implementations of Diffie-Hellman, RSA, DSS, and other systems},
  author={Kocher, Paul C},
  booktitle={Advances in Cryptology—CRYPTO’96: 16th Annual International Cryptology Conference Santa Barbara, California, USA August 18--22, 1996 Proceedings 16},
  pages={104--113},
  year={1996},
  organization={Springer}
}

@article{yarom2017cachebleed,
  title={CacheBleed: a timing attack on OpenSSL constant-time RSA},
  author={Yarom, Yuval and Genkin, Daniel and Heninger, Nadia},
  journal={Journal of Cryptographic Engineering},
  volume={7},
  pages={99--112},
  year={2017},
  publisher={Springer}
}

@article{moghimi2019memjam,
  title={Memjam: A false dependency attack against constant-time crypto implementations},
  author={Moghimi, Ahmad and Wichelmann, Jan and Eisenbarth, Thomas and Sunar, Berk},
  journal={International Journal of Parallel Programming},
  volume={47},
  pages={538--570},
  year={2019},
  publisher={Springer}
}

@inproceedings{gullasch2011cache,
  title={Cache games--bringing access-based cache attacks on AES to practice},
  author={Gullasch, David and Bangerter, Endre and Krenn, Stephan},
  booktitle={2011 IEEE Symposium on Security and Privacy},
  pages={490--505},
  year={2011},
  organization={IEEE}
}

@article{tromer2010efficient,
  title={Efficient cache attacks on AES, and countermeasures},
  author={Tromer, Eran and Osvik, Dag Arne and Shamir, Adi},
  journal={Journal of Cryptology},
  volume={23},
  pages={37--71},
  year={2010},
  publisher={Springer}
}

@article{bernstein2005cache,
  title={Cache-timing attacks on AES},
  author={Bernstein, Daniel J},
  year={2005}
}

@inproceedings{wang2017cached,
  title={$\{$CacheD$\}$: Identifying $\{$Cache-Based$\}$ timing channels in production software},
  author={Wang, Shuai and Wang, Pei and Liu, Xiao and Zhang, Danfeng and Wu, Dinghao},
  booktitle={26th USENIX security symposium (USENIX security 17)},
  pages={235--252},
  year={2017}
}

@inproceedings{felten2000timing,
  title={Timing attacks on web privacy},
  author={Felten, Edward W and Schneider, Michael A},
  booktitle={Proceedings of the 7th ACM Conference on Computer and Communications Security},
  pages={25--32},
  year={2000}
}

@inproceedings{oren2015spy,
  title={The spy in the sandbox: Practical cache attacks in javascript and their implications},
  author={Oren, Yossef and Kemerlis, Vasileios P and Sethumadhavan, Simha and Keromytis, Angelos D},
  booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
  pages={1406--1418},
  year={2015}
}

@inproceedings{brumley2011remote,
  title={Remote timing attacks are still practical},
  author={Brumley, Billy Bob and Tuveri, Nicola},
  booktitle={European Symposium on Research in Computer Security},
  pages={355--371},
  year={2011},
  organization={Springer}
}

@misc{percival2005cache,
  title={Cache missing for fun and profit},
  author={Percival, Colin},
  year={2005},
  publisher={BSDCan Ottawa}
}

@inproceedings{gruss2019page,
  title={Page cache attacks},
  author={Gruss, Daniel and Kraft, Erik and Tiwari, Trishita and Schwarz, Michael and Trachtenberg, Ari and Hennessey, Jason and Ionescu, Alex and Fogh, Anders},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={167--180},
  year={2019}
}

@inproceedings{pessl2016drama,
  title={$\{$DRAMA$\}$: Exploiting $\{$DRAM$\}$ addressing for $\{$Cross-CPU$\}$ attacks},
  author={Pessl, Peter and Gruss, Daniel and Maurice, Cl{\'e}mentine and Schwarz, Michael and Mangard, Stefan},
  booktitle={25th USENIX security symposium (USENIX security 16)},
  pages={565--581},
  year={2016}
}

@inproceedings{van2020timeless,
  title={Timeless timing attacks: Exploiting concurrency to leak secrets over remote connections},
  author={Van Goethem, Tom and P{\"o}pper, Christina and Joosen, Wouter and Vanhoef, Mathy},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={1985--2002},
  year={2020}
}

@inproceedings{jattke2022blacksmith,
  title={Blacksmith: Scalable rowhammering in the frequency domain},
  author={Jattke, Patrick and Van Der Veen, Victor and Frigo, Pietro and Gunter, Stijn and Razavi, Kaveh},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={716--734},
  year={2022},
  organization={IEEE}
}

@inproceedings{jattke2024zenhammer,
  title={Zenhammer: Rowhammer attacks on amd zen-based platforms},
  author={Jattke, Patrick and Wipfli, Max and Solt, Flavien and Marazzi, Michele and B{\"o}lcskei, Matej and Razavi, Kaveh},
  booktitle={33rd USENIX Security Symposium (USENIX Security 2024)},
  year={2024}
}
@inproceedings{schwarz2017fantastic,
  title={Fantastic timers and where to find them: High-resolution microarchitectural attacks in JavaScript},
  author={Schwarz, Michael and Maurice, Cl{\'e}mentine and Gruss, Daniel and Mangard, Stefan},
  booktitle={Financial Cryptography and Data Security: 21st International Conference, FC 2017, Sliema, Malta, April 3-7, 2017, Revised Selected Papers 21},
  pages={247--267},
  year={2017},
  organization={Springer}
}

@inproceedings{evtyushkin2016jump,
  title={Jump over ASLR: Attacking branch predictors to bypass ASLR},
  author={Evtyushkin, Dmitry and Ponomarev, Dmitry and Abu-Ghazaleh, Nael},
  booktitle={2016 49th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={1--13},
  year={2016},
  organization={IEEE}
}

@inproceedings{gruss2017kaslr,
  title={Kaslr is dead: long live kaslr},
  author={Gruss, Daniel and Lipp, Moritz and Schwarz, Michael and Fellner, Richard and Maurice, Cl{\'e}mentine and Mangard, Stefan},
  booktitle={Engineering Secure Software and Systems: 9th International Symposium, ESSoS 2017, Bonn, Germany, July 3-5, 2017, Proceedings 9},
  pages={161--176},
  year={2017},
  organization={Springer}
}

@inproceedings{lin2024peep,
  title={Peep With A Mirror: Breaking The Integrity of Android App Sandboxing via Unprivileged Cache Side Channel},
  author={Lin, Yan and Wong, Joshua and Li, Xiang and Ma, Haoyu and Gao, Debin},
  booktitle={33rd USENIX Security Symposium (USENIX Security 24)},
  pages={2119--2135},
  year={2024}
}

@inproceedings{irazoqui2015s,
  title={S \$ A: A shared cache attack that works across cores and defies VM sandboxing--and its application to AES},
  author={Irazoqui, Gorka and Eisenbarth, Thomas and Sunar, Berk},
  booktitle={2015 IEEE Symposium on Security and Privacy},
  pages={591--604},
  year={2015},
  organization={IEEE}
}

@inproceedings{barresi2015cain,
  title={$\{$CAIN$\}$: Silently breaking $\{$ASLR$\}$ in the cloud},
  author={Barresi, Antonio and Razavi, Kaveh and Payer, Mathias and Gross, Thomas R},
  booktitle={9th USENIX Workshop on Offensive Technologies (WOOT 15)},
  year={2015}
}

@inproceedings{lindemann2018memory,
  title={A memory-deduplication side-channel attack to detect applications in co-resident virtual machines},
  author={Lindemann, Jens and Fischer, Mathias},
  booktitle={Proceedings of the 33rd Annual ACM Symposium on Applied Computing},
  pages={183--192},
  year={2018}
}

@article{schwarzl2021remote,
  title={Remote memory-deduplication attacks},
  author={Schwarzl, Martin and Kraft, Erik and Lipp, Moritz and Gruss, Daniel},
  journal={arXiv preprint arXiv:2111.08553},
  year={2021}
}

@article{kim2021breaking,
  title={Breaking KASLR using memory deduplication in virtualized environments},
  author={Kim, Taehun and Kim, Taehyun and Shin, Youngjoo},
  journal={Electronics},
  volume={10},
  number={17},
  pages={2174},
  year={2021},
  publisher={MDPI}
}

@article{suzaki2013implementation,
  title={Implementation of a memory disclosure attack on memory deduplication of virtual machines},
  author={Suzaki, Kuniyasu and Iijima, Kengo and Yagi, Toshiki and Artho, Cyrille},
  journal={IEICE TRANSACTIONS on Fundamentals of Electronics, Communications and Computer Sciences},
  volume={96},
  number={1},
  pages={215--224},
  year={2013},
  publisher={The Institute of Electronics, Information and Communication Engineers}
}

@inproceedings{suzaki2011memory,
  title={Memory deduplication as a threat to the guest OS},
  author={Suzaki, Kuniyasu and Iijima, Kengo and Yagi, Toshiki and Artho, Cyrille},
  booktitle={Proceedings of the Fourth European Workshop on System Security},
  pages={1--6},
  year={2011}
}

@inproceedings{bosman2016dedup,
  title={Dedup est machina: Memory deduplication as an advanced exploitation vector},
  author={Bosman, Erik and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={2016 IEEE symposium on security and privacy (SP)},
  pages={987--1004},
  year={2016},
  organization={IEEE}
}


@inproceedings{hund2013practical,
  title={Practical timing side channel attacks against kernel space ASLR},
  author={Hund, Ralf and Willems, Carsten and Holz, Thorsten},
  booktitle={2013 IEEE Symposium on Security and Privacy},
  pages={191--205},
  year={2013},
  organization={IEEE}
}

@article{ojha2020timing,
  title={Timing Cache Accesses to Eliminate Side Channels in Shared Software},
  author={Ojha, Divya and Dwarkadas, Sandhya},
  journal={arXiv preprint arXiv:2009.14732},
  year={2020}
}

@inproceedings{frigo2020trrespass,
  title={TRRespass: Exploiting the many sides of target row refresh},
  author={Frigo, Pietro and Vannacc, Emanuele and Hassan, Hasan and Van Der Veen, Victor and Mutlu, Onur and Giuffrida, Cristiano and Bos, Herbert and Razavi, Kaveh},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={747--762},
  year={2020},
  organization={IEEE}
}

@inproceedings{dessouky2020hybcache,
  title={$\{$HybCache$\}$: Hybrid $\{$Side-Channel-Resilient$\}$ caches for trusted execution environments},
  author={Dessouky, Ghada and Frassetto, Tommaso and Sadeghi, Ahmad-Reza},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={451--468},
  year={2020}
}

@article{gras2018tlbleed,
  title={Tlbleed: When protecting your cpu caches is not enough},
  author={Gras, B and Razavi, KAVEH and Bos, H and Giuffrida, C},
  journal={Black Hat},
  year={2018}
}

@inproceedings{kwong2020rambleed,
  title={Rambleed: Reading bits in memory without accessing them},
  author={Kwong, Andrew and Genkin, Daniel and Gruss, Daniel and Yarom, Yuval},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={695--711},
  year={2020},
  organization={IEEE}
}

@inproceedings{naghibijouybari2018rendered,
  title={Rendered insecure: Gpu side channel attacks are practical},
  author={Naghibijouybari, Hoda and Neupane, Ajaya and Qian, Zhiyun and Abu-Ghazaleh, Nael},
  booktitle={Proceedings of the 2018 ACM SIGSAC conference on computer and communications security},
  pages={2139--2153},
  year={2018}
}

@inproceedings{gruss2016rowhammer,
  title={Rowhammer. js: A remote software-induced fault attack in javascript},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Mangard, Stefan},
  booktitle={Detection of Intrusions and Malware, and Vulnerability Assessment: 13th International Conference, DIMVA 2016, San Sebasti{\'a}n, Spain, July 7-8, 2016, Proceedings 13},
  pages={300--321},
  year={2016},
  organization={Springer}
}

@inproceedings{tatar2018throwhammer,
  title={Throwhammer: Rowhammer attacks over the network and defenses},
  author={Tatar, Andrei and Konoth, Radhesh Krishnan and Athanasopoulos, Elias and Giuffrida, Cristiano and Bos, Herbert and Razavi, Kaveh},
  booktitle={2018 USENIX Annual Technical Conference (USENIX ATC 18)},
  pages={213--226},
  year={2018}
}

@inproceedings{cohen2022hammerscope,
  title={Hammerscope: Observing dram power consumption using rowhammer},
  author={Cohen, Yaakov and Tharayil, Kevin Sam and Haenel, Arie and Genkin, Daniel and Keromytis, Angelos D and Oren, Yossi and Yarom, Yuval},
  booktitle={Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security},
  pages={547--561},
  year={2022}
}

@inproceedings{qiao2016new,
  title={A new approach for rowhammer attacks},
  author={Qiao, Rui and Seaborn, Mark},
  booktitle={2016 IEEE international symposium on hardware oriented security and trust (HOST)},
  pages={161--166},
  year={2016},
  organization={IEEE}
}

@article{halderman2009lest,
  title={Lest we remember: cold-boot attacks on encryption keys},
  author={Halderman, J Alex and Schoen, Seth D and Heninger, Nadia and Clarkson, William and Paul, William and Calandrino, Joseph A and Feldman, Ariel J and Appelbaum, Jacob and Felten, Edward W},
  journal={Communications of the ACM},
  volume={52},
  number={5},
  pages={91--98},
  year={2009},
  publisher={ACM New York, NY, USA}
}
@article{guo2022don,
  title={Don’t reject this: Key-recovery timing attacks due to rejection-sampling in HQC and BIKE},
  author={Guo, Qian and Hlauschek, Clemens and Johansson, Thomas and Lahr, Norman and Nilsson, Alexander and Schr{\"o}der, Robin Leander},
  journal={IACR Transactions on Cryptographic Hardware and Embedded Systems},
  pages={223--263},
  year={2022}
}

@inproceedings{zimerman2021recovering,
  title={Recovering AES Keys with a Deep Cold Boot Attack},
  author={Zimerman, Itamar and Nachmani, Eliya and Wolf, Lior},
  booktitle={International Conference on Machine Learning},
  pages={12955--12966},
  year={2021},
  organization={PMLR}
}

@article{villanueva2020cold,
  title={Cold boot attacks on LUOV},
  author={Villanueva-Polanco, Ricardo},
  journal={Applied Sciences},
  volume={10},
  number={12},
  pages={4106},
  year={2020},
  publisher={MDPI}
}

@article{wetzels2014hidden,
  title={Hidden in snow, revealed in thaw: Cold boot attacks revisited},
  author={Wetzels, Jos},
  journal={arXiv preprint arXiv:1408.0725},
  year={2014}
}

@inproceedings{luo2023rowpress,
  title={Rowpress: Amplifying read disturbance in modern dram chips},
  author={Luo, Haocong and Olgun, Ataberk and Ya{\u{g}}l{\i}k{\c{c}}{\i}, Abdullah Giray and Tu{\u{g}}rul, Yahya Can and Rhyner, Steve and Cavlak, Meryem Banu and Lindegger, Jo{\"e}l and Sadrosadati, Mohammad and Mutlu, Onur},
  booktitle={Proceedings of the 50th Annual International Symposium on Computer Architecture},
  pages={1--18},
  year={2023}
}

@inproceedings{zeitouni2018s,
  title={It's hammer time: how to attack (rowhammer-based) DRAM-PUFs},
  author={Zeitouni, Shaza and Gens, David and Sadeghi, Ahmad-Reza},
  booktitle={Proceedings of the 55th Annual Design Automation Conference},
  pages={1--6},
  year={2018}
}

@inproceedings{hassan2016chargecache,
  title={ChargeCache: Reducing DRAM latency by exploiting row access locality},
  author={Hassan, Hasan and Pekhimenko, Gennady and Vijaykumar, Nandita and Seshadri, Vivek and Lee, Donghyuk and Ergin, Oguz and Mutlu, Onur},
  booktitle={2016 IEEE International Symposium on High Performance Computer Architecture (HPCA)},
  pages={581--593},
  year={2016},
  organization={IEEE}
}

@inproceedings{li2021cipherleaks,
  title={$\{$CIPHERLEAKS$\}$: Breaking Constant-time Cryptography on $\{$AMD$\}$$\{$SEV$\}$ via the Ciphertext Side Channel},
  author={Li, Mengyuan and Zhang, Yinqian and Wang, Huibo and Li, Kang and Cheng, Yueqiang},
  booktitle={30th USENIX Security Symposium (USENIX Security 21)},
  pages={717--732},
  year={2021}
}

@inproceedings{wang2023nvleak,
  title={$\{$NVLeak$\}$:$\{$Off-Chip$\}$$\{$Side-Channel$\}$ Attacks via $\{$Non-Volatile$\}$ Memory Systems},
  author={Wang, Zixuan and Taram, Mohammadkazem and Moghimi, Daniel and Swanson, Steven and Tullsen, Dean and Zhao, Jishen},
  booktitle={32nd USENIX Security Symposium (USENIX Security 23)},
  pages={6771--6788},
  year={2023}
}

@inproceedings{baviskar2024cache,
  title={Cache Based Side-Channel Attacks: A Survey},
  author={Baviskar, Swapnil and Sanoj, R and Nath, Hiran V},
  booktitle={2024 IEEE Recent Advances in Intelligent Computational Systems (RAICS)},
  pages={1--8},
  year={2024},
  organization={IEEE}
}

@article{su2021survey,
  title={Survey of CPU Cache-Based Side-Channel Attacks: Systematic Analysis, Security Models, and Countermeasures},
  author={Su, Chao and Zeng, Qingkai},
  journal={Security and Communication Networks},
  volume={2021},
  number={1},
  pages={5559552},
  year={2021},
  publisher={Wiley Online Library}
}

@article{wang2023side,
  title={Side-channel attack analysis on in-memory computing architectures},
  author={Wang, Ziyu and Meng, Fan-hsuan and Park, Yongmo and Eshraghian, Jason K and Lu, Wei D},
  journal={IEEE Transactions on Emerging Topics in Computing},
  volume={12},
  number={1},
  pages={109--121},
  year={2023},
  publisher={IEEE}
}

@article{anwar2017cross,
  title={Cross-VM cache-based side channel attacks and proposed prevention mechanisms: A survey},
  author={Anwar, Shahid and Inayat, Zakira and Zolkipli, Mohamad Fadli and Zain, Jasni Mohamad and Gani, Abdullah and Anuar, Nor Badrul and Khan, Muhammad Khurram and Chang, Victor},
  journal={Journal of Network and Computer Applications},
  volume={93},
  pages={259--279},
  year={2017},
  publisher={Elsevier}
}

@article{lyu2018survey,
  title={A survey of side-channel attacks on caches and countermeasures},
  author={Lyu, Yangdi and Mishra, Prabhat},
  journal={Journal of Hardware and Systems Security},
  volume={2},
  pages={33--50},
  year={2018},
  publisher={Springer}
}

@article{lou2021survey,
  title={A survey of microarchitectural side-channel vulnerabilities, attacks, and defenses in cryptography},
  author={Lou, Xiaoxuan and Zhang, Tianwei and Jiang, Jun and Zhang, Yinqian},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--37},
  year={2021},
  publisher={ACM New York, NY, USA}
}



@inproceedings{kogler2022half,
  title={Half-Double\$: Hammering from the next row over},
  author={Kogler, Andreas and Juffinger, Jonas and Qazi, Salman and Kim, Yoongu and Lipp, Moritz and Boichat, Nicolas and Shiu, Eric and Nissler, Mattias and Gruss, Daniel},
  booktitle={31st USENIX Security Symposium (USENIX Security 22)},
  pages={3807--3824},
  year={2022}
}

=======================================

@inproceedings{liu2015last,
  title={Last-level cache side-channel attacks are practical},
  author={Liu, Fangfei and Yarom, Yuval and Ge, Qian and Heiser, Gernot and Lee, Ruby B},
  booktitle={2015 IEEE symposium on security and privacy},
  pages={605--622},
  year={2015},
  organization={IEEE}
}

@inproceedings{yarom2014flush+,
  title={$\{$FLUSH+ RELOAD$\}$: A high resolution, low noise, l3 cache $\{$Side-Channel$\}$ attack},
  author={Yarom, Yuval and Falkner, Katrina},
  booktitle={23rd USENIX security symposium (USENIX security 14)},
  pages={719--732},
  year={2014}
}

@inproceedings{gras2018translation,
  title={Translation leak-aside buffer: Defeating cache side-channel protections with $\{$TLB$\}$ attacks},
  author={Gras, Ben and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={955--972},
  year={2018}
}

@inproceedings{wang2017leaky,
  title={Leaky cauldron on the dark land: Understanding memory side-channel hazards in SGX},
  author={Wang, Wenhao and Chen, Guoxing and Pan, Xiaorui and Zhang, Yinqian and Wang, XiaoFeng and Bindschaedler, Vincent and Tang, Haixu and Gunter, Carl A},
  booktitle={Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security},
  pages={2421--2434},
  year={2017}
}

@inproceedings{schwarzl2023practical,
  title={Practical timing side-channel attacks on memory compression},
  author={Schwarzl, Martin and Borrello, Pietro and Saileshwar, Gururaj and M{\"u}ller, Hanna and Schwarz, Michael and Gruss, Daniel},
  booktitle={2023 IEEE Symposium on Security and Privacy (SP)},
  pages={1186--1203},
  year={2023},
  organization={IEEE}
}

@inproceedings{schwarz2017fantastic,
  title={Fantastic timers and where to find them: High-resolution microarchitectural attacks in JavaScript},
  author={Schwarz, Michael and Maurice, Cl{\'e}mentine and Gruss, Daniel and Mangard, Stefan},
  booktitle={Financial Cryptography and Data Security: 21st International Conference, FC 2017, Sliema, Malta, April 3-7, 2017, Revised Selected Papers 21},
  pages={247--267},
  year={2017},
  organization={Springer}
}

@article{kocher2020spectre,
  title={Spectre attacks: Exploiting speculative execution},
  author={Kocher, Paul and Horn, Jann and Fogh, Anders and Genkin, Daniel and Gruss, Daniel and Haas, Werner and Hamburg, Mike and Lipp, Moritz and Mangard, Stefan and Prescher, Thomas and others},
  journal={Communications of the ACM},
  volume={63},
  number={7},
  pages={93--101},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{kocher2020spectre,
  title={Spectre attacks: Exploiting speculative execution},
  author={Kocher, Paul and Horn, Jann and Fogh, Anders and Genkin, Daniel and Gruss, Daniel and Haas, Werner and Hamburg, Mike and Lipp, Moritz and Mangard, Stefan and Prescher, Thomas and others},
  journal={Communications of the ACM},
  volume={63},
  number={7},
  pages={93--101},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{lipp2020meltdown,
  title={Meltdown: Reading kernel memory from user space},
  author={Lipp, Moritz and Schwarz, Michael and Gruss, Daniel and Prescher, Thomas and Haas, Werner and Horn, Jann and Mangard, Stefan and Kocher, Paul and Genkin, Daniel and Yarom, Yuval and others},
  journal={Communications of the ACM},
  volume={63},
  number={6},
  pages={46--56},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@inproceedings{bhattacharyya2019smotherspectre,
  title={Smotherspectre: exploiting speculative execution through port contention},
  author={Bhattacharyya, Atri and Sandulescu, Alexandra and Neugschwandtner, Matthias and Sorniotti, Alessandro and Falsafi, Babak and Payer, Mathias and Kurmus, Anil},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={785--800},
  year={2019}
}

@inproceedings{islam2019spoiler,
  title={$\{$SPOILER$\}$: Speculative load hazards boost rowhammer and cache attacks},
  author={Islam, Saad and Moghimi, Ahmad and Bruhns, Ida and Krebbel, Moritz and Gulmezoglu, Berk and Eisenbarth, Thomas and Sunar, Berk},
  booktitle={28th USENIX Security Symposium (USENIX Security 19)},
  pages={621--637},
  year={2019}
}

@inproceedings{koruyeh2018spectre,
  title={Spectre returns! speculation attacks using the return stack buffer},
  author={Koruyeh, Esmaeil Mohammadian and Khasawneh, Khaled N and Song, Chengyu and Abu-Ghazaleh, Nael},
  booktitle={12th USENIX Workshop on Offensive Technologies (WOOT 18)},
  year={2018}
}

@inproceedings{wikner2022retbleed,
  title={$\{$RETBLEED$\}$: Arbitrary speculative code execution with return instructions},
  author={Wikner, Johannes and Razavi, Kaveh},
  booktitle={31st USENIX Security Symposium (USENIX Security 22)},
  pages={3825--3842},
  year={2022}
}

@inproceedings{trujillo2023inception,
  title={Inception: Exposing new attack surfaces with training in transient execution},
  author={Trujillo, Dani{\"e}l and Wikner, Johannes and Razavi, Kaveh},
  booktitle={32nd USENIX Security Symposium (USENIX Security 23)},
  pages={7303--7320},
  year={2023}
}

@inproceedings{shen2024specrun,
  title={SPECRUN: The Danger of Speculative Runahead Execution in Processors},
  author={Shen, Chaoqun and Qu, Gang and Zhang, Jiliang},
  booktitle={Proceedings of the 61st ACM/IEEE Design Automation Conference},
  pages={1--6},
  year={2024}
}

@article{chowdhuryy2021leaking,
  title={Leaking secrets through modern branch predictors in the speculative world},
  author={Chowdhuryy, Md Hafizul Islam and Yao, Fan},
  journal={IEEE Transactions on Computers},
  volume={71},
  number={9},
  pages={2059--2072},
  year={2021},
  publisher={IEEE}
}

@inproceedings{ragab2024ghostrace,
  title={GhostRace: Exploiting and Mitigating Speculative Race Conditions},
  author={Ragab, Hany and Mambretti, Andrea and Kurmus, Anil and Giuffrida, Cristiano},
  booktitle={USENIX Security},
  year={2024}
}

@article{kim2024tiktag,
  title={TikTag: Breaking ARM's Memory Tagging Extension with Speculative Execution},
  author={Kim, Juhee and Park, Jinbum and Roh, Sihyeon and Chung, Jaeyoung and Lee, Youngjoo and Kim, Taesoo and Lee, Byoungyoung},
  journal={arXiv preprint arXiv:2406.08719},
  year={2024}
}

@inproceedings{li2024indirector,
  title={Indirector:$\{$High-Precision$\}$ Branch Target Injection Attacks Exploiting the Indirect Branch Predictor},
  author={Li, Luyi and Yavarzadeh, Hosein and Tullsen, Dean},
  booktitle={33rd USENIX Security Symposium (USENIX Security 24)},
  pages={2137--2154},
  year={2024}
}

@inproceedings{van2021cacheout,
  title={CacheOut: Leaking data on Intel CPUs via cache evictions},
  author={Van Schaik, Stephan and Minkin, Marina and Kwong, Andrew and Genkin, Daniel and Yarom, Yuval},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={339--354},
  year={2021},
  organization={IEEE}
}

@article{dall2018cachequote,
  title={Cachequote: Efficiently recovering long-term secrets of SGX EPID via cache attacks},
  author={Dall, Fergus and De Micheli, Gabrielle and Eisenbarth, Thomas and Genkin, Daniel and Heninger, Nadia and Moghimi, Ahmad and Yarom, Yuval},
  year={2018},
  publisher={IACR Transactions on Cryptographic Hardware and Embedded Systems}
}

@inproceedings{canella2019fallout,
  title={Fallout: Leaking data on meltdown-resistant cpus},
  author={Canella, Claudio and Genkin, Daniel and Giner, Lukas and Gruss, Daniel and Lipp, Moritz and Minkin, Marina and Moghimi, Daniel and Piessens, Frank and Schwarz, Michael and Sunar, Berk and others},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={769--784},
  year={2019}
}

@article{yarom2017cachebleed,
  title={CacheBleed: a timing attack on OpenSSL constant-time RSA},
  author={Yarom, Yuval and Genkin, Daniel and Heninger, Nadia},
  journal={Journal of Cryptographic Engineering},
  volume={7},
  pages={99--112},
  year={2017},
  publisher={Springer}
}

@inproceedings{gruss2015cache,
  title={Cache template attacks: Automating attacks on inclusive $\{$Last-Level$\}$ caches},
  author={Gruss, Daniel and Spreitzer, Raphael and Mangard, Stefan},
  booktitle={24th USENIX Security Symposium (USENIX Security 15)},
  pages={897--912},
  year={2015}
}

@inproceedings{liu2015last,
  title={Last-level cache side-channel attacks are practical},
  author={Liu, Fangfei and Yarom, Yuval and Ge, Qian and Heiser, Gernot and Lee, Ruby B},
  booktitle={2015 IEEE symposium on security and privacy},
  pages={605--622},
  year={2015},
  organization={IEEE}
}

@inproceedings{shusterman2021prime+,
  title={$\{$Prime+ Probe$\}$ 1,$\{$JavaScript$\}$ 0: Overcoming Browser-based $\{$Side-Channel$\}$ Defenses},
  author={Shusterman, Anatoly and Agarwal, Ayush and O'Connell, Sioli and Genkin, Daniel and Oren, Yossi and Yarom, Yuval},
  booktitle={30th USENIX Security Symposium (USENIX Security 21)},
  pages={2863--2880},
  year={2021}
}

@inproceedings{hund2013practical,
  title={Practical timing side channel attacks against kernel space ASLR},
  author={Hund, Ralf and Willems, Carsten and Holz, Thorsten},
  booktitle={2013 IEEE Symposium on Security and Privacy},
  pages={191--205},
  year={2013},
  organization={IEEE}
}

@inproceedings{gras2017aslr,
  title={ASLR on the Line: Practical Cache Attacks on the MMU.},
  author={Gras, Ben and Razavi, Kaveh and Bosman, Erik and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={NDSS},
  volume={17},
  pages={26},
  year={2017}
}

@inproceedings{gruss2019page,
  title={Page cache attacks},
  author={Gruss, Daniel and Kraft, Erik and Tiwari, Trishita and Schwarz, Michael and Trachtenberg, Ari and Hennessey, Jason and Ionescu, Alex and Fogh, Anders},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={167--180},
  year={2019}
}

@inproceedings{disselkoen2017prime+,
  title={$\{$Prime+ Abort$\}$: A $\{$Timer-Free$\}$$\{$High-Precision$\}$ L3 Cache Attack using Intel $\{$TSX$\}$},
  author={Disselkoen, Craig and Kohlbrenner, David and Porter, Leo and Tullsen, Dean},
  booktitle={26th USENIX Security Symposium (USENIX Security 17)},
  pages={51--67},
  year={2017}
}

@inproceedings{oren2015spy,
  title={The spy in the sandbox: Practical cache attacks in javascript and their implications},
  author={Oren, Yossef and Kemerlis, Vasileios P and Sethumadhavan, Simha and Keromytis, Angelos D},
  booktitle={Proceedings of the 22nd ACM SIGSAC Conference on Computer and Communications Security},
  pages={1406--1418},
  year={2015}
}

@inproceedings{aciiccmez2007yet,
  title={Yet another microarchitectural attack: exploiting I-cache},
  author={Acii{\c{c}}mez, Onur},
  booktitle={Proceedings of the 2007 ACM workshop on Computer security architecture},
  pages={11--18},
  year={2007}
}

@inproceedings{van2017telling,
  title={Telling your secrets without page faults: Stealthy page $\{$Table-Based$\}$ attacks on enclaved execution},
  author={Van Bulck, Jo and Weichbrodt, Nico and Kapitza, R{\"u}diger and Piessens, Frank and Strackx, Raoul},
  booktitle={26th USENIX Security Symposium (USENIX Security 17)},
  pages={1041--1056},
  year={2017}
}

@inproceedings{yan2020cache,
  title={Cache telepathy: Leveraging shared resource attacks to learn $\{$DNN$\}$ architectures},
  author={Yan, Mengjia and Fletcher, Christopher W and Torrellas, Josep},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={2003--2020},
  year={2020}
}

@inproceedings{zhang2012cross,
  title={Cross-VM side channels and their use to extract private keys},
  author={Zhang, Yinqian and Juels, Ari and Reiter, Michael K and Ristenpart, Thomas},
  booktitle={Proceedings of the 2012 ACM conference on Computer and communications security},
  pages={305--316},
  year={2012}
}

@inproceedings{gruss2016prefetch,
  title={Prefetch side-channel attacks: Bypassing SMAP and kernel ASLR},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Fogh, Anders and Lipp, Moritz and Mangard, Stefan},
  booktitle={Proceedings of the 2016 ACM SIGSAC conference on computer and communications security},
  pages={368--379},
  year={2016}
}

@inproceedings{kemerlis2014ret2dir,
  title={ret2dir: Rethinking kernel isolation},
  author={Kemerlis, Vasileios P and Polychronakis, Michalis and Keromytis, Angelos D},
  booktitle={23rd USENIX Security Symposium (USENIX Security 14)},
  pages={957--972},
  year={2014}
}

@inproceedings{wang2017leaky,
  title={Leaky cauldron on the dark land: Understanding memory side-channel hazards in SGX},
  author={Wang, Wenhao and Chen, Guoxing and Pan, Xiaorui and Zhang, Yinqian and Wang, XiaoFeng and Bindschaedler, Vincent and Tang, Haixu and Gunter, Carl A},
  booktitle={Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security},
  pages={2421--2434},
  year={2017}
}

@inproceedings{xu2015controlled,
  title={Controlled-channel attacks: Deterministic side channels for untrusted operating systems},
  author={Xu, Yuanzhong and Cui, Weidong and Peinado, Marcus},
  booktitle={2015 IEEE Symposium on Security and Privacy},
  pages={640--656},
  year={2015},
  organization={IEEE}
}

@inproceedings{yan2020cache,
  title={Cache telepathy: Leveraging shared resource attacks to learn $\{$DNN$\}$ architectures},
  author={Yan, Mengjia and Fletcher, Christopher W and Torrellas, Josep},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={2003--2020},
  year={2020}
}

@inproceedings{van2017telling,
  title={Telling your secrets without page faults: Stealthy page $\{$Table-Based$\}$ attacks on enclaved execution},
  author={Van Bulck, Jo and Weichbrodt, Nico and Kapitza, R{\"u}diger and Piessens, Frank and Strackx, Raoul},
  booktitle={26th USENIX Security Symposium (USENIX Security 17)},
  pages={1041--1056},
  year={2017}
}

@inproceedings{gras2018translation,
  title={Translation leak-aside buffer: Defeating cache side-channel protections with $\{$TLB$\}$ attacks},
  author={Gras, Ben and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={955--972},
  year={2018}
}

@inproceedings{deng2020benchmark,
  title={A benchmark suite for evaluating caches' vulnerability to timing attacks},
  author={Deng, Shuwen and Xiong, Wenjie and Szefer, Jakub},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={683--697},
  year={2020}
}

@article{deng2021evaluation,
  title={Evaluation of cache attacks on arm processors and secure caches},
  author={Deng, Shuwen and Matyunin, Nikolay and Xiong, Wenjie and Katzenbeisser, Stefan and Szefer, Jakub},
  journal={IEEE Transactions on Computers},
  volume={71},
  number={9},
  pages={2248--2262},
  year={2021},
  publisher={IEEE}
}

@article{briongos2020cache,
  title={CACHE SNIPER: Accurate timing control of cache evictions},
  author={Briongos, Samira and Bruhns, Ida and Malag{\'o}n, Pedro and Eisenbarth, Thomas and Moya, Jos{\'e} M},
  journal={arXiv preprint arXiv:2008.12188},
  year={2020}
}

@article{zhang2014cache,
  title={Cache-based Side-Channel Attacks in Multi-Tenant Public Clouds and Their Countermeasures},
  author={Zhang, Yinqian},
  year={2014},
  publisher={University of North Carolina at Chapel Hill Graduate School}
}

@inproceedings{schwarzl2023practical,
  title={Practical timing side-channel attacks on memory compression},
  author={Schwarzl, Martin and Borrello, Pietro and Saileshwar, Gururaj and M{\"u}ller, Hanna and Schwarz, Michael and Gruss, Daniel},
  booktitle={2023 IEEE Symposium on Security and Privacy (SP)},
  pages={1186--1203},
  year={2023},
  organization={IEEE}
}

@inproceedings{van2016drammer,
  title={Drammer: Deterministic rowhammer attacks on mobile platforms},
  author={Van Der Veen, Victor and Fratantonio, Yanick and Lindorfer, Martina and Gruss, Daniel and Maurice, Cl{\'e}mentine and Vigna, Giovanni and Bos, Herbert and Razavi, Kaveh and Giuffrida, Cristiano},
  booktitle={Proceedings of the 2016 ACM SIGSAC conference on computer and communications security},
  pages={1675--1689},
  year={2016}
}

@article{kim2014flipping,
  title={Flipping bits in memory without accessing them: An experimental study of DRAM disturbance errors},
  author={Kim, Yoongu and Daly, Ross and Kim, Jeremie and Fallin, Chris and Lee, Ji Hye and Lee, Donghyuk and Wilkerson, Chris and Lai, Konrad and Mutlu, Onur},
  journal={ACM SIGARCH Computer Architecture News},
  volume={42},
  number={3},
  pages={361--372},
  year={2014},
  publisher={ACM New York, NY, USA}
}

@inproceedings{bhattacharya2016curious,
  title={Curious case of rowhammer: flipping secret exponent bits using timing analysis},
  author={Bhattacharya, Sarani and Mukhopadhyay, Debdeep},
  booktitle={Cryptographic Hardware and Embedded Systems--CHES 2016: 18th International Conference, Santa Barbara, CA, USA, August 17-19, 2016, Proceedings 18},
  pages={602--624},
  year={2016},
  organization={Springer}
}

@inproceedings{schwarz2017fantastic,
  title={Fantastic timers and where to find them: High-resolution microarchitectural attacks in JavaScript},
  author={Schwarz, Michael and Maurice, Cl{\'e}mentine and Gruss, Daniel and Mangard, Stefan},
  booktitle={Financial Cryptography and Data Security: 21st International Conference, FC 2017, Sliema, Malta, April 3-7, 2017, Revised Selected Papers 21},
  pages={247--267},
  year={2017},
  organization={Springer}
}

@inproceedings{van2020timeless,
  title={Timeless timing attacks: Exploiting concurrency to leak secrets over remote connections},
  author={Van Goethem, Tom and P{\"o}pper, Christina and Joosen, Wouter and Vanhoef, Mathy},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={1985--2002},
  year={2020}
}

@article{cheng2024evict+,
  title={Evict+ Spec+ Time: Exploiting Out-of-Order Execution to Improve Cache-Timing Attacks},
  author={Cheng, Shing Hing William and Chuengsatiansup, Chitchanok and Genkin, Daniel and McNeil, Dallas and Murray, Toby and Yarom, Yuval and Zhang, Zhiyuan},
  journal={Cryptology ePrint Archive},
  year={2024}
}

@article{jin2023timing,
  title={Timing the Transient Execution: A New Side-Channel Attack on Intel CPUs},
  author={Jin, Yu and Qiu, Pengfei and Wang, Chunlu and Yang, Yihao and Wang, Dongsheng and Qu, Gang},
  journal={arXiv preprint arXiv:2304.10877},
  year={2023}
}

@inproceedings{xiao2023hacky,
  title={Hacky racers: Exploiting instruction-level parallelism to generate stealthy fine-grained timers},
  author={Xiao, Haocheng and Ainsworth, Sam},
  booktitle={Proceedings of the 28th ACM International Conference on Architectural Support for Programming Languages and Operating Systems, Volume 2},
  pages={354--369},
  year={2023}
}

@inproceedings{kholoosi2023empirical,
  title={Empirical Analysis of Software Vulnerabilities Causing Timing Side Channels},
  author={Kholoosi, M Mehdi and Babar, M Ali and Yilmaz, Cemal},
  booktitle={2023 IEEE Conference on Communications and Network Security (CNS)},
  pages={1--9},
  year={2023},
  organization={IEEE}
}

@inproceedings{suzaki2011software,
  title={Software side channel attack on memory deduplication},
  author={Suzaki, Kuniyasu and Iijima, Kengo and Yagi, Toshiki and Artho, Cyrille},
  booktitle={ACM Symposium on Operating Systems Principles (SOSP 2011), Poster session},
  year={2011}
}

@inproceedings{evtyushkin2016jump,
  title={Jump over ASLR: Attacking branch predictors to bypass ASLR},
  author={Evtyushkin, Dmitry and Ponomarev, Dmitry and Abu-Ghazaleh, Nael},
  booktitle={2016 49th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={1--13},
  year={2016},
  organization={IEEE}
}

@inproceedings{lee2017inferring,
  title={Inferring fine-grained control flow inside $\{$SGX$\}$ enclaves with branch shadowing},
  author={Lee, Sangho and Shih, Ming-Wei and Gera, Prasun and Kim, Taesoo and Kim, Hyesoon and Peinado, Marcus},
  booktitle={26th USENIX Security Symposium (USENIX Security 17)},
  pages={557--574},
  year={2017}
}

@article{evtyushkin2018branchscope,
  title={Branchscope: A new side-channel attack on directional branch predictor},
  author={Evtyushkin, Dmitry and Riley, Ryan and Abu-Ghazaleh, Nael CSE and ECE and Ponomarev, Dmitry},
  journal={ACM SIGPLAN Notices},
  volume={53},
  number={2},
  pages={693--707},
  year={2018},
  publisher={ACM New York, NY, USA}
}

@article{gras2018tlbleed,
  title={Tlbleed: When protecting your cpu caches is not enough},
  author={Gras, B and Razavi, KAVEH and Bos, H and Giuffrida, C},
  journal={Black Hat},
  year={2018}
}

@article{weisse2018foreshadow,
  title={Foreshadow-NG: Breaking the virtual memory abstraction with transient out-of-order execution},
  author={Weisse, Ofir and Van Bulck, Jo and Minkin, Marina and Genkin, Daniel and Kasikci, Baris and Piessens, Frank and Silberstein, Mark and Strackx, Raoul and Wenisch, Thomas F and Yarom, Yuval},
  year={2018}
}

@inproceedings{van2018foreshadow,
  title={Foreshadow: Extracting the keys to the intel $\{$SGX$\}$ kingdom with transient $\{$Out-of-Order$\}$ execution},
  author={Van Bulck, Jo and Minkin, Marina and Weisse, Ofir and Genkin, Daniel and Kasikci, Baris and Piessens, Frank and Silberstein, Mark and Wenisch, Thomas F and Yarom, Yuval and Strackx, Raoul},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={991--1008},
  year={2018}
}

@inproceedings{koruyeh2018spectre,
  title={Spectre returns! speculation attacks using the return stack buffer},
  author={Koruyeh, Esmaeil Mohammadian and Khasawneh, Khaled N and Song, Chengyu and Abu-Ghazaleh, Nael},
  booktitle={12th USENIX Workshop on Offensive Technologies (WOOT 18)},
  year={2018}
}

@inproceedings{van2019ridl,
  title={RIDL: Rogue in-flight data load},
  author={Van Schaik, Stephan and Milburn, Alyssa and {\"O}sterlund, Sebastian and Frigo, Pietro and Maisuradze, Giorgi and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={88--105},
  year={2019},
  organization={IEEE}
}

@inproceedings{schwarz2019zombieload,
  title={ZombieLoad: Cross-privilege-boundary data sampling},
  author={Schwarz, Michael and Lipp, Moritz and Moghimi, Daniel and Van Bulck, Jo and Stecklina, Julian and Prescher, Thomas and Gruss, Daniel},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={753--768},
  year={2019}
}

@inproceedings{chen2019sgxpectre,
  title={Sgxpectre: Stealing intel secrets from sgx enclaves via speculative execution},
  author={Chen, Guoxing and Chen, Sanchuan and Xiao, Yuan and Zhang, Yinqian and Lin, Zhiqiang and Lai, Ten H},
  booktitle={2019 IEEE European Symposium on Security and Privacy (EuroS\&P)},
  pages={142--157},
  year={2019},
  organization={IEEE}
}

@inproceedings{murdock2020plundervolt,
  title={Plundervolt: Software-based fault injection attacks against Intel SGX},
  author={Murdock, Kit and Oswald, David and Garcia, Flavio D and Van Bulck, Jo and Gruss, Daniel and Piessens, Frank},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={1466--1482},
  year={2020},
  organization={IEEE}
}

@inproceedings{cui2021smashex,
  title={Smashex: Smashing sgx enclaves using exceptions},
  author={Cui, Jinhua and Yu, Jason Zhijingcheng and Shinde, Shweta and Saxena, Prateek and Cai, Zhiping},
  booktitle={Proceedings of the 2021 ACM SIGSAC conference on computer and communications security},
  pages={779--793},
  year={2021}
}

@article{sridhara2024sigy,
  title={SIGY: Breaking Intel SGX Enclaves with Malicious Exceptions \& Signals},
  author={Sridhara, Supraja and Bertschi, Andrin and Schl{\"u}ter, Benedict and Shinde, Shweta},
  journal={arXiv preprint arXiv:2404.13998},
  year={2024}
}

@inproceedings{cloosters2020teerex,
  title={$\{$TeeRex$\}$: Discovery and exploitation of memory corruption vulnerabilities in $\{$SGX$\}$ enclaves},
  author={Cloosters, Tobias and Rodler, Michael and Davi, Lucas},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={841--858},
  year={2020}
}

@misc{flippingpages2024,
  author       = {Notselwyn},
  title        = {Flipping Pages: An analysis of a new Linux vulnerability in nf\_tables and hardened exploitation techniques},
  year         = {2024},
  howpublished = {\url{https://pwning.tech/nftables/}},
  note         = {Accessed: [Insert Date Here]}
}

@inproceedings{wicherski2013,
  author       = {Georg Wicherski and Alexandru Radocea},
  title        = {Hacking like in the Movies: Visualizing Page Tables for Local Exploitation},
  booktitle    = {Black Hat USA},
  year         = {2013},
  howpublished = {\url{https://media.blackhat.com/us-13/US-13-Wicherski-Hacking-like-in-the-Movies-Visualizing-Page-Tables-WP.pdf}},
  note         = {Accessed: [Insert Date Here]}
}


@article{yoshioka2024gbhammer,
  title={GbHammer: Malicious Inter-process Page Sharing by Hammering Global Bits in Page Table Entries},
  author={Yoshioka, Keigo and Akiyama, Soramichi},
  journal={arXiv preprint arXiv:2406.13119},
  year={2024}
}

@inproceedings{li2021crossline,
  title={Crossline: Breaking" security-by-crash" based memory isolation in amd sev},
  author={Li, Mengyuan and Zhang, Yinqian and Lin, Zhiqiang},
  booktitle={Proceedings of the 2021 ACM SIGSAC Conference on Computer and Communications Security},
  pages={2937--2950},
  year={2021}
}

@inproceedings{moghimi2020copycat,
  title={$\{$CopyCat$\}$: Controlled $\{$Instruction-Level$\}$ attacks on enclaves},
  author={Moghimi, Daniel and Van Bulck, Jo and Heninger, Nadia and Piessens, Frank and Sunar, Berk},
  booktitle={29th USENIX security symposium (USENIX security 20)},
  pages={469--486},
  year={2020}
}

@article{parida2021pagedumper,
  title={PageDumper: a mechanism to collect page table manipulation information at run-time},
  author={Parida, Trushna and Das, Suvrojit},
  journal={International Journal of Information Security},
  volume={20},
  pages={603--619},
  year={2021},
  publisher={Springer}
}

@inproceedings{barresi2015cain,
  title={$\{$CAIN$\}$: Silently breaking $\{$ASLR$\}$ in the cloud},
  author={Barresi, Antonio and Razavi, Kaveh and Payer, Mathias and Gross, Thomas R},
  booktitle={9th USENIX Workshop on Offensive Technologies (WOOT 15)},
  year={2015}
}

@inproceedings{lindemann2018memory,
  title={A memory-deduplication side-channel attack to detect applications in co-resident virtual machines},
  author={Lindemann, Jens and Fischer, Mathias},
  booktitle={Proceedings of the 33rd Annual ACM Symposium on Applied Computing},
  pages={183--192},
  year={2018}
}

@article{schwarzl2021remote,
  title={Remote memory-deduplication attacks},
  author={Schwarzl, Martin and Kraft, Erik and Lipp, Moritz and Gruss, Daniel},
  journal={arXiv preprint arXiv:2111.08553},
  year={2021}
}

@article{kim2021breaking,
  title={Breaking KASLR using memory deduplication in virtualized environments},
  author={Kim, Taehun and Kim, Taehyun and Shin, Youngjoo},
  journal={Electronics},
  volume={10},
  number={17},
  pages={2174},
  year={2021},
  publisher={MDPI}
}

@article{suzaki2013implementation,
  title={Implementation of a memory disclosure attack on memory deduplication of virtual machines},
  author={Suzaki, Kuniyasu and Iijima, Kengo and Yagi, Toshiki and Artho, Cyrille},
  journal={IEICE TRANSACTIONS on Fundamentals of Electronics, Communications and Computer Sciences},
  volume={96},
  number={1},
  pages={215--224},
  year={2013},
  publisher={The Institute of Electronics, Information and Communication Engineers}
}

@inproceedings{bosman2016dedup,
  title={Dedup est machina: Memory deduplication as an advanced exploitation vector},
  author={Bosman, Erik and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={2016 IEEE symposium on security and privacy (SP)},
  pages={987--1004},
  year={2016},
  organization={IEEE}
}

@book{mangard2008power,
  title={Power analysis attacks: Revealing the secrets of smart cards},
  author={Mangard, Stefan and Oswald, Elisabeth and Popp, Thomas},
  volume={31},
  year={2008},
  publisher={Springer Science \& Business Media}
}

@inproceedings{kocher1999differential,
  title={Differential power analysis},
  author={Kocher, P},
  booktitle={Proc. Advances in Cryptology (CRYPTO'99)},
  year={1999}
}

@inproceedings{hutter2014temperature,
  title={The temperature side channel and heating fault attacks},
  author={Hutter, Michael and Schmidt, J{\"o}rn-Marc},
  booktitle={Smart Card Research and Advanced Applications: 12th International Conference, CARDIS 2013, Berlin, Germany, November 27-29, 2013. Revised Selected Papers 12},
  pages={219--235},
  year={2014},
  organization={Springer}
}

@inproceedings{agrawal2003multi,
  title={Multi-channel attacks},
  author={Agrawal, Dakshi and Rao, Josyula R and Rohatgi, Pankaj},
  booktitle={Cryptographic Hardware and Embedded Systems-CHES 2003: 5th International Workshop, Cologne, Germany, September 8--10, 2003. Proceedings 5},
  pages={2--16},
  year={2003},
  organization={Springer}
}

@inproceedings{brier2004correlation,
  title={Correlation power analysis with a leakage model},
  author={Brier, Eric and Clavier, Christophe and Olivier, Francis},
  booktitle={Cryptographic Hardware and Embedded Systems-CHES 2004: 6th International Workshop Cambridge, MA, USA, August 11-13, 2004. Proceedings 6},
  pages={16--29},
  year={2004},
  organization={Springer}
}

@article{srivastava2024scar,
  title={SCAR: Power Side-Channel Analysis at RTL Level},
  author={Srivastava, Amisha and Das, Sanjay and Choudhury, Navnil and Psiakis, Rafail and Silva, Pedro Henrique and Pal, Debjit and Basu, Kanad},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  year={2024},
  publisher={IEEE}
}

@article{liao2020security,
  title={Security analysis of IoT devices by using mobile computing: a systematic literature review},
  author={Liao, Bin and Ali, Yasir and Nazir, Shah and He, Long and Khan, Habib Ullah},
  journal={IEEE Access},
  volume={8},
  pages={120331--120350},
  year={2020},
  publisher={IEEE}
}

@article{chawla2023power,
  title={The Power of Telemetry: Uncovering Software-Based Side-Channel Attacks on Apple M1/M2 Systems},
  author={Chawla, Nikhil and Liu, Chen and Chakraborty, Abhishek and Chervatyuk, Igor and Sun, Ke and Hamasaki, Thais Moreira and Kawakami, Henrique},
  journal={arXiv preprint arXiv:2306.16391},
  year={2023}
}


@inproceedings{batina2019csi,
  title={$\{$CSI$\}$$\{$NN$\}$: Reverse engineering of neural network architectures through electromagnetic side channel},
  author={Batina, Lejla and Bhasin, Shivam and Jap, Dirmanto and Picek, Stjepan},
  booktitle={28th USENIX Security Symposium (USENIX Security 19)},
  pages={515--532},
  year={2019}
}

@article{bronchain2021give,
  title={Give me 5 minutes: Attacking ASCAD with a single side-channel trace},
  author={Bronchain, Olivier and Cassiers, Ga{\"e}tan and Standaert, Fran{\c{c}}ois-Xavier},
  journal={Cryptology ePrint Archive},
  year={2021}
}

@inproceedings{das2019x,
  title={X-DeepSCA: Cross-device deep learning side channel attack},
  author={Das, Debayan and Golder, Anupam and Danial, Josef and Ghosh, Santosh and Raychowdhury, Arijit and Sen, Shreyas},
  booktitle={Proceedings of the 56th Annual Design Automation Conference 2019},
  pages={1--6},
  year={2019}
}

@article{oflynn2018can,
  author    = {Colin O'Flynn and Greg d'Eon},
  title     = {Power Analysis and Fault Attacks against Secure CAN: How Safe Are Your Keys?},
  journal   = {SAE International Journal of Transportation Cybersecurity and Privacy},
  volume    = {1},
  number    = {1},
  pages     = {5-16},
  year      = {2018},
  doi       = {10.4271/11-01-01-0001},
  url       = {https://www.researchgate.net/publication/324242120_Power_Analysis_and_Fault_Attacks_against_Secure_CAN_How_Safe_Are_Your_Keys}
}

@article{kim2022thermalbleed,
  title={Thermalbleed: A practical thermal side-channel attack},
  author={Kim, Taehun and Shin, Youngjoo},
  journal={IEEE Access},
  volume={10},
  pages={25718--25731},
  year={2022},
  publisher={IEEE}
}

@inproceedings{zhang2024thermalscope,
  title={ThermalScope: A Practical Interrupt Side Channel Attack Based on Thermal Event Interrupts},
  author={Zhang, Xin and Zhang, Zhi and Shen, Qingni and Wang, Wenhao and Gao, Yansong and Yang, Zhuoxi and Wu, Zhonghai},
  booktitle={Proceedings of the 61st ACM/IEEE Design Automation Conference},
  pages={1--6},
  year={2024}
}

@article{kim2022thermalbleed,
  title={Thermalbleed: A practical thermal side-channel attack},
  author={Kim, Taehun and Shin, Youngjoo},
  journal={IEEE Access},
  volume={10},
  pages={25718--25731},
  year={2022},
  publisher={IEEE}
}

@article{aljuffri2021applying,
  title={Applying thermal side-channel attacks on asymmetric cryptography},
  author={Aljuffri, Abdullah and Zwalua, Marc and Reinbrecht, Cezar Rodolfo Wedig and Hamdioui, Said and Taouil, Mottaqiallah},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={29},
  number={11},
  pages={1930--1942},
  year={2021},
  publisher={IEEE}
}

@inproceedings{bekaert2022thermal,
  title={Are thermal attacks a realistic threat? Investigating the preconditions of thermal attacks in users’ daily lives},
  author={Bekaert, Paul and Alotaibi, Norah and Mathis, Florian and Gerber, Nina and Rafferty, Aidan Christopher and Khamis, Mohamed and Marky, Karola},
  booktitle={Nordic Human-Computer Interaction Conference},
  pages={1--9},
  year={2022}
}

@inproceedings{liu2019side,
  title={Side channel attacks in computation offloading systems with gpu virtualization},
  author={Liu, Sihang and Wei, Yizhou and Chi, Jianfeng and Shezan, Faysal Hossain and Tian, Yuan},
  booktitle={2019 IEEE Security and Privacy Workshops (SPW)},
  pages={156--161},
  year={2019},
  organization={IEEE}
}

@article{benelhaouare2024mitigating,
  title={Mitigating Thermal Side-Channel Vulnerabilities in FPGA-Based SiP Systems Through Advanced Thermal Management and Security Integration Using Thermal Digital Twin (TDT) Technology},
  author={Benelhaouare, Amrou Zyad and Mellal, Idir and Oumlaz, Maroua and Lakhssassi, Ahmed},
  journal={Electronics},
  volume={13},
  number={21},
  pages={4176},
  year={2024},
  publisher={MDPI}
}

@inproceedings{zhang2024thermalscope,
  title={ThermalScope: A Practical Interrupt Side Channel Attack Based on Thermal Event Interrupts},
  author={Zhang, Xin and Zhang, Zhi and Shen, Qingni and Wang, Wenhao and Gao, Yansong and Yang, Zhuoxi and Wu, Zhonghai},
  booktitle={Proceedings of the 61st ACM/IEEE Design Automation Conference},
  pages={1--6},
  year={2024}
}

@inproceedings{agrawal2003side,
  title={The EM side—channel (s)},
  author={Agrawal, Dakshi and Archambeault, Bruce and Rao, Josyula R and Rohatgi, Pankaj},
  booktitle={Cryptographic Hardware and Embedded Systems-CHES 2002: 4th International Workshop Redwood Shores, CA, USA, August 13--15, 2002 Revised Papers 4},
  pages={29--45},
  year={2003},
  organization={Springer}
}

@inproceedings{genkin2016ecdh,
  title={ECDH key-extraction via low-bandwidth electromagnetic attacks on PCs},
  author={Genkin, Daniel and Pachmanov, Lev and Pipman, Itamar and Tromer, Eran},
  booktitle={Topics in Cryptology-CT-RSA 2016: The Cryptographers' Track at the RSA Conference 2016, San Francisco, CA, USA, February 29-March 4, 2016, Proceedings},
  pages={219--235},
  year={2016},
  organization={Springer}
}

@inproceedings{heyszl2012localized,
  title={Localized electromagnetic analysis of cryptographic implementations},
  author={Heyszl, Johann and Mangard, Stefan and Heinz, Benedikt and Stumpf, Frederic and Sigl, Georg},
  booktitle={Topics in Cryptology--CT-RSA 2012: The Cryptographers’ Track at the RSA Conference 2012, San Francisco, CA, USA, February 27--March 2, 2012. Proceedings},
  pages={231--244},
  year={2012},
  organization={Springer}
}

@inproceedings{wang2022hertzbleed,
  title={Hertzbleed: Turning power $\{$Side-Channel$\}$ attacks into remote timing attacks on x86},
  author={Wang, Yingchen and Paccagnella, Riccardo and He, Elizabeth Tang and Shacham, Hovav and Fletcher, Christopher W and Kohlbrenner, David},
  booktitle={31st USENIX Security Symposium (USENIX Security 22)},
  pages={679--697},
  year={2022}
}

@article{sayakkara2019leveraging,
  title={Leveraging electromagnetic side-channel analysis for the investigation of IoT devices},
  author={Sayakkara, Asanka and Le-Khac, Nhien-An and Scanlon, Mark},
  journal={Digital Investigation},
  volume={29},
  pages={S94--S103},
  year={2019},
  publisher={Elsevier}
}

@article{danial2021x,
  title={Em-x-dl: Efficient cross-device deep learning side-channel attack with noisy em signatures},
  author={Danial, Josef and Das, Debayan and Golder, Anupam and Ghosh, Santosh and Raychowdhury, Arijit and Sen, Shreyas},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={18},
  number={1},
  pages={1--17},
  year={2021},
  publisher={ACM New York, NY}
}

@article{das2020electromagnetic,
  title={Electromagnetic and power side-channel analysis: Advanced attacks and low-overhead generic countermeasures through white-box approach},
  author={Das, Debayan and Sen, Shreyas},
  journal={Cryptography},
  volume={4},
  number={4},
  pages={30},
  year={2020},
  publisher={MDPI}
}

@article{kinugawa2017evaluation,
  title={Evaluation of EM information leakage caused by IEMI with hardware trojan},
  author={Kinugawa, Masahiro and Hayashi, Yu Ichi and Mori, Tatsuya},
  journal={IEEJ Transactions on Fundamentals and Materials},
  volume={137},
  number={3},
  pages={153--157},
  year={2017},
  publisher={The Institute of Electrical Engineers of Japan}
}

@inproceedings{yu2020deepem,
  title={Deepem: Deep neural networks model recovery through em side-channel information leakage},
  author={Yu, Honggang and Ma, Haocheng and Yang, Kaichen and Zhao, Yiqiang and Jin, Yier},
  booktitle={2020 IEEE International Symposium on Hardware Oriented Security and Trust (HOST)},
  pages={209--218},
  year={2020},
  organization={IEEE}
}

@article{mutlu2019rowhammer,
  title={Rowhammer: A retrospective},
  author={Mutlu, Onur and Kim, Jeremie S},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={8},
  pages={1555--1571},
  year={2019},
  publisher={IEEE}
}

@inproceedings{frigo2020trrespass,
  title={TRRespass: Exploiting the many sides of target row refresh},
  author={Frigo, Pietro and Vannacc, Emanuele and Hassan, Hasan and Van Der Veen, Victor and Mutlu, Onur and Giuffrida, Cristiano and Bos, Herbert and Razavi, Kaveh},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={747--762},
  year={2020},
  organization={IEEE}
}

@article{halderman2009lest,
  title={Lest we remember: cold-boot attacks on encryption keys},
  author={Halderman, J Alex and Schoen, Seth D and Heninger, Nadia and Clarkson, William and Paul, William and Calandrino, Joseph A and Feldman, Ariel J and Appelbaum, Jacob and Felten, Edward W},
  journal={Communications of the ACM},
  volume={52},
  number={5},
  pages={91--98},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{markettos2019thunderclap,
  title={Thunderclap: Exploring vulnerabilities in operating system IOMMU protection via DMA from untrustworthy peripherals},
  author={Markettos, A Theodore and Rothwell, Colin and Gutstein, Brett F and Pearce, Allison and Neumann, Peter G and Moore, Simon W and Watson, Robert NM},
  year={2019},
  publisher={Internet Society}
}

@article{de2023forensic,
  title={Forensic method for decrypting TPM-protected BitLocker volumes using Intel DCI},
  author={de Assump{\c{c}}{\~a}o, Matheus Bichara and dos Reis, Marcelo Abdalla and Marcondes, Marcos Roberto and da Silva Eleut{\'e}rio, Pedro Monteiro and Vieira, Victor Hugo},
  journal={Forensic Science International: Digital Investigation},
  volume={44},
  pages={301514},
  year={2023},
  publisher={Elsevier}
}

@inproceedings{jattke2022blacksmith,
  title={Blacksmith: Scalable rowhammering in the frequency domain},
  author={Jattke, Patrick and Van Der Veen, Victor and Frigo, Pietro and Gunter, Stijn and Razavi, Kaveh},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={716--734},
  year={2022},
  organization={IEEE}
}
@inproceedings{jattke2024zenhammer,
  title={Zenhammer: Rowhammer attacks on amd zen-based platforms},
  author={Jattke, Patrick and Wipfli, Max and Solt, Flavien and Marazzi, Michele and B{\"o}lcskei, Matej and Razavi, Kaveh},
  booktitle={33rd USENIX Security Symposium (USENIX Security 2024)},
  year={2024}
}
@inproceedings{gruss2016rowhammer,
  title={Rowhammer. js: A remote software-induced fault attack in javascript},
  author={Gruss, Daniel and Maurice, Cl{\'e}mentine and Mangard, Stefan},
  booktitle={Detection of Intrusions and Malware, and Vulnerability Assessment: 13th International Conference, DIMVA 2016, San Sebasti{\'a}n, Spain, July 7-8, 2016, Proceedings 13},
  pages={300--321},
  year={2016},
  organization={Springer}
}

@inproceedings{tatar2018throwhammer,
  title={Throwhammer: Rowhammer attacks over the network and defenses},
  author={Tatar, Andrei and Konoth, Radhesh Krishnan and Athanasopoulos, Elias and Giuffrida, Cristiano and Bos, Herbert and Razavi, Kaveh},
  booktitle={2018 USENIX Annual Technical Conference (USENIX ATC 18)},
  pages={213--226},
  year={2018}
}

@inproceedings{cohen2022hammerscope,
  title={Hammerscope: Observing dram power consumption using rowhammer},
  author={Cohen, Yaakov and Tharayil, Kevin Sam and Haenel, Arie and Genkin, Daniel and Keromytis, Angelos D and Oren, Yossi and Yarom, Yuval},
  booktitle={Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security},
  pages={547--561},
  year={2022}
}
@inproceedings{qiao2016new,
  title={A new approach for rowhammer attacks},
  author={Qiao, Rui and Seaborn, Mark},
  booktitle={2016 IEEE international symposium on hardware oriented security and trust (HOST)},
  pages={161--166},
  year={2016},
  organization={IEEE}
}

@inproceedings{bhattacharyya2019smotherspectre,
  title={Smotherspectre: exploiting speculative execution through port contention},
  author={Bhattacharyya, Atri and Sandulescu, Alexandra and Neugschwandtner, Matthias and Sorniotti, Alessandro and Falsafi, Babak and Payer, Mathias and Kurmus, Anil},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={785--800},
  year={2019}
}

@inproceedings{kwong2020rambleed,
  title={Rambleed: Reading bits in memory without accessing them},
  author={Kwong, Andrew and Genkin, Daniel and Gruss, Daniel and Yarom, Yuval},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={695--711},
  year={2020},
  organization={IEEE}
}

@inproceedings{won2021deepfreeze,
  title={Deepfreeze: Cold boot attacks and high fidelity model recovery on commercial edgeml device},
  author={Won, Yoo-Seung and Chatterjee, Soham and Jap, Dirmanto and Basu, Arindam and Bhasin, Shivam},
  booktitle={2021 IEEE/ACM International Conference On Computer Aided Design (ICCAD)},
  pages={1--9},
  year={2021},
  organization={IEEE}
}

@article{banegas2023recovering,
  title={On recovering block cipher secret keys in the cold boot attack setting},
  author={Banegas, Gustavo and Villanueva-Polanco, Ricardo},
  journal={Cryptography and Communications},
  pages={1--25},
  year={2023},
  publisher={Springer}
}

@article{villanueva2020cold,
  title={Cold boot attacks on LUOV},
  author={Villanueva-Polanco, Ricardo},
  journal={Applied Sciences},
  volume={10},
  number={12},
  pages={4106},
  year={2020},
  publisher={MDPI}
}

@inproceedings{zimerman2021recovering,
  title={Recovering AES Keys with a Deep Cold Boot Attack},
  author={Zimerman, Itamar and Nachmani, Eliya and Wolf, Lior},
  booktitle={International Conference on Machine Learning},
  pages={12955--12966},
  year={2021},
  organization={PMLR}
}

@article{wetzels2014hidden,
  title={Hidden in snow, revealed in thaw: Cold boot attacks revisited},
  author={Wetzels, Jos},
  journal={arXiv preprint arXiv:1408.0725},
  year={2014}
}

@article{frisk2016direct,
  title={Direct memory attack the kernel},
  author={Frisk, Ulf},
  journal={Proceedings of DEFCON},
  volume={24},
  year={2016}
}

@article{frisk18pcileech,
  title={PCILeech--GitHub, 2021},
  author={Frisk, Ulf},
  journal={URL https://github. com/ufrisk/pcileech.[Last Accessed: June 18, 2021]}
}

@inproceedings{matsuo2024smmpack,
  title={SmmPack: Obfuscation for SMM Modules with TPM Sealed Key},
  author={Matsuo, Kazuki and Tanda, Satoshi and Suzaki, Kuniyasu and Kawakoya, Yuhei and Mori, Tatsuya},
  booktitle={International Conference on Detection of Intrusions and Malware, and Vulnerability Assessment},
  pages={439--459},
  year={2024},
  organization={Springer}
}

@inproceedings{butterworth2013bios,
  title={Bios chronomancy: Fixing the core root of trust for measurement},
  author={Butterworth, John and Kallenberg, Corey and Kovah, Xeno and Herzog, Amy},
  booktitle={Proceedings of the 2013 ACM SIGSAC conference on Computer \& Communications Security},
  pages={25--36},
  year={2013}
}

@inproceedings{tan2021invisible,
  title={Invisible probe: Timing attacks with PCIe congestion side-channel},
  author={Tan, Mingtian and Wan, Junpeng and Zhou, Zhe and Li, Zhou},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={322--338},
  year={2021},
  organization={IEEE}
}

@inproceedings{van2017sgx,
  title={SGX-Step: A practical attack framework for precise enclave execution control},
  author={Van Bulck, Jo and Piessens, Frank and Strackx, Raoul},
  booktitle={Proceedings of the 2nd Workshop on System Software for Trusted Execution},
  pages={1--6},
  year={2017}
}

@inproceedings{ali2021connoc,
  title={ConNOC: A practical timing channel attack on network-on-chip hardware in a multicore processor},
  author={Ali, Usman and Khan, Omer},
  booktitle={2021 IEEE International Symposium on Hardware Oriented Security and Trust (HOST)},
  pages={192--202},
  year={2021},
  organization={IEEE}
}

@inproceedings{dutta2021leaky,
  title={Leaky buddies: Cross-component covert channels on integrated CPU-GPU systems},
  author={Dutta, Sankha Baran and Naghibijouybari, Hoda and Abu-Ghazaleh, Nael and Marquez, Andres and Barker, Kevin},
  booktitle={2021 ACM/IEEE 48th Annual International Symposium on Computer Architecture (ISCA)},
  pages={972--984},
  year={2021},
  organization={IEEE}
}

@inproceedings{chen2024bridge,
  title={Bridge and hint: Extending pre-trained language models for long-range code},
  author={Chen, Yujia and Gao, Cuiyun and Yang, Zezhou and Zhang, Hongyu and Liao, Qing},
  booktitle={Proceedings of the 33rd ACM SIGSOFT International Symposium on Software Testing and Analysis},
  pages={274--286},
  year={2024}
}

@inproceedings{gruss2017kaslr,
  title={Kaslr is dead: long live kaslr},
  author={Gruss, Daniel and Lipp, Moritz and Schwarz, Michael and Fellner, Richard and Maurice, Cl{\'e}mentine and Mangard, Stefan},
  booktitle={Engineering Secure Software and Systems: 9th International Symposium, ESSoS 2017, Bonn, Germany, July 3-5, 2017, Proceedings 9},
  pages={161--176},
  year={2017},
  organization={Springer}
}

@inproceedings{irazoqui2015s,
  title={S \$ A: A shared cache attack that works across cores and defies VM sandboxing--and its application to AES},
  author={Irazoqui, Gorka and Eisenbarth, Thomas and Sunar, Berk},
  booktitle={2015 IEEE Symposium on Security and Privacy},
  pages={591--604},
  year={2015},
  organization={IEEE}
}

@inproceedings{guo2022adversarial,
  title={Adversarial prefetch: New cross-core cache side channel attacks},
  author={Guo, Yanan and Zigerelli, Andrew and Zhang, Youtao and Yang, Jun},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={1458--1473},
  year={2022},
  organization={IEEE}
}

@inproceedings{lin2024peep,
  title={Peep With A Mirror: Breaking The Integrity of Android App Sandboxing via Unprivileged Cache Side Channel},
  author={Lin, Yan and Wong, Joshua and Li, Xiang and Ma, Haoyu and Gao, Debin},
  booktitle={33rd USENIX Security Symposium (USENIX Security 24)},
  pages={2119--2135},
  year={2024}
}

@article{moghimi2019memjam,
  title={Memjam: A false dependency attack against constant-time crypto implementations},
  author={Moghimi, Ahmad and Wichelmann, Jan and Eisenbarth, Thomas and Sunar, Berk},
  journal={International Journal of Parallel Programming},
  volume={47},
  pages={538--570},
  year={2019},
  publisher={Springer}
}

@inproceedings{dai2022don,
  title={Don't mesh around:$\{$Side-Channel$\}$ attacks and mitigations on mesh interconnects},
  author={Dai, Miles and Paccagnella, Riccardo and Gomez-Garcia, Miguel and McCalpin, John and Yan, Mengjia},
  booktitle={31st USENIX Security Symposium (USENIX Security 22)},
  pages={2857--2874},
  year={2022}
}

@article{chacon2021coherence,
  title={Coherence Attacks and Countermeasures in Interposer-Based Systems},
  author={Chacon, Gino and Mandal, Tapojyoti and Knechtel, Johann and Sinanoglu, Ozgur and Gratz, Paul and Soteriou, Vassos},
  journal={arXiv preprint arXiv:2105.02917},
  year={2021}
}

@inproceedings{mustafa2023covert,
  title={Covert Communication Attacks in Chiplet-based 2.5-D Integration Systems},
  author={Mustafa, Yerzhan and K{\"o}se, Sel{\c{c}}uk},
  booktitle={2023 IEEE 36th International System-on-Chip Conference (SOCC)},
  pages={1--5},
  year={2023},
  organization={IEEE}
}

@article{zhang2024beyond,
  title={Beyond the Bridge: Contention-Based Covert and Side Channel Attacks on Multi-GPU Interconnect},
  author={Zhang, Yicheng and Nazaraliyev, Ravan and Dutta, Sankha Baran and Abu-Ghazaleh, Nael and Marquez, Andres and Barker, Kevin},
  journal={arXiv preprint arXiv:2404.03877},
  year={2024}
}

@inproceedings{paccagnella2021lord,
  title={Lord of the ring (s): Side channel attacks on the $\{$CPU$\}$$\{$On-Chip$\}$ ring interconnect are practical},
  author={Paccagnella, Riccardo and Luo, Licheng and Fletcher, Christopher W},
  booktitle={30th USENIX Security Symposium (USENIX Security 21)},
  pages={645--662},
  year={2021}
}

@inproceedings{jin2024ghost,
  title={Ghost Arbitration: Mitigating Interconnect Side-Channel Timing Attacks in GPU},
  author={Jin, Zhixian and Ahn, Jaeguk and Kim, Jiho and Kasan, Hans and Song, Jina and Song, Wonjun and Kim, John},
  booktitle={2024 57th IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={1138--1152},
  year={2024},
  organization={IEEE}
}

@book{lee2022building,
  title={Building Trusted Execution Environments},
  author={Lee, Dayeol},
  year={2022},
  publisher={University of California, Berkeley}
}

@inproceedings{savino2024multicore,
  title={Multicore DRAM Bank-\& Row-Conflict Bomb for Timing Attacks in Mixed-Criticality Systems},
  author={Savino, Antonio and Gala, Gautam and Cinque, Marcello and Fohler, Gerhard},
  booktitle={2024 IEEE 27th International Symposium on Real-Time Distributed Computing (ISORC)},
  pages={1--10},
  year={2024},
  organization={IEEE}
}

@inproceedings{bechtel2023cache,
  title={Cache bank-aware denial-of-service attacks on multicore ARM processors},
  author={Bechtel, Michael and Yun, Heechul},
  booktitle={2023 IEEE 29th Real-Time and Embedded Technology and Applications Symposium (RTAS)},
  pages={198--208},
  year={2023},
  organization={IEEE}
}

@inproceedings{naghibijouybari2018rendered,
  title={Rendered insecure: Gpu side channel attacks are practical},
  author={Naghibijouybari, Hoda and Neupane, Ajaya and Qian, Zhiyun and Abu-Ghazaleh, Nael},
  booktitle={Proceedings of the 2018 ACM SIGSAC conference on computer and communications security},
  pages={2139--2153},
  year={2018}
}

@inproceedings{dutta2023spy,
  title={Spy in the GPU-box: Covert and side channel attacks on multi-GPU systems},
  author={Dutta, Sankha Baran and Naghibijouybari, Hoda and Gupta, Arjun and Abu-Ghazaleh, Nael and Marquez, Andres and Barker, Kevin},
  booktitle={Proceedings of the 50th Annual International Symposium on Computer Architecture},
  pages={1--13},
  year={2023}
}

@inproceedings{karimi2020hardware,
  title={Hardware/software obfuscation against timing side-channel attack on a GPU},
  author={Karimi, Elmira and Fei, Yunsi and Kaeli, David},
  booktitle={2020 IEEE International Symposium on Hardware Oriented Security and Trust (HOST)},
  pages={122--131},
  year={2020},
  organization={IEEE}
}

@inproceedings{ferguson2024webgpu,
  title={Webgpu-spy: Finding fingerprints in the sandbox through gpu cache attacks},
  author={Ferguson, Ethan and Wilson, Adam and Naghibijouybari, Hoda},
  booktitle={Proceedings of the 19th ACM Asia Conference on Computer and Communications Security},
  pages={158--171},
  year={2024}
}

@inproceedings{giner2024generic,
  title={Generic and Automated Drive-by GPU Cache Attacks from the Browser},
  author={Giner, Lukas and Czerny, Roland and Gruber, Christoph and Rauscher, Fabian and Kogler, Andreas and Braga, Daniel De Almeida and Gruss, Daniel},
  booktitle={Proceedings of the 19th ACM Asia Conference on Computer and Communications Security},
  pages={128--140},
  year={2024}
}

@inproceedings{cronin2021exploration,
  title={An exploration of ARM system-level cache and GPU side channels},
  author={Cronin, Patrick and Gao, Xing and Wang, Haining and Cotton, Chase},
  booktitle={Proceedings of the 37th Annual Computer Security Applications Conference},
  pages={784--795},
  year={2021}
}

@inproceedings{side2022lockeddown,
  title={Lockeddown: Exploiting contention on host-gpu pcie bus for fun and profit},
  author={Side, Mert and Yao, Fan and Zhang, Zhenkai},
  booktitle={2022 IEEE 7th European Symposium on Security and Privacy (EuroS\&P)},
  pages={270--285},
  year={2022},
  organization={IEEE}
}

@inproceedings{liu2016catalyst,
  title={Catalyst: Defeating last-level cache side channel attacks in cloud computing},
  author={Liu, Fangfei and Ge, Qian and Yarom, Yuval and Mckeen, Frank and Rozas, Carlos and Heiser, Gernot and Lee, Ruby B},
  booktitle={2016 IEEE international symposium on high performance computer architecture (HPCA)},
  pages={406--418},
  year={2016},
  organization={IEEE}
}

@inproceedings{werner2019scattercache,
  title={$\{$ScatterCache$\}$: thwarting cache attacks via cache set randomization},
  author={Werner, Mario and Unterluggauer, Thomas and Giner, Lukas and Schwarz, Michael and Gruss, Daniel and Mangard, Stefan},
  booktitle={28th USENIX Security Symposium (USENIX Security 19)},
  pages={675--692},
  year={2019}
}

@inproceedings{kiriansky2018dawg,
  title={DAWG: A defense against cache timing attacks in speculative execution processors},
  author={Kiriansky, Vladimir and Lebedev, Ilia and Amarasinghe, Saman and Devadas, Srinivas and Emer, Joel},
  booktitle={2018 51st Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={974--987},
  year={2018},
  organization={IEEE}
}

@inproceedings{gruss2017strong,
  title={Strong and efficient cache $\{$Side-Channel$\}$ protection using hardware transactional memory},
  author={Gruss, Daniel and Lettner, Julian and Schuster, Felix and Ohrimenko, Olya and Haller, Istvan and Costa, Manuel},
  booktitle={26th USENIX Security Symposium (USENIX Security 17)},
  pages={217--233},
  year={2017}
}

@inproceedings{chen2018racing,
  title={Racing in hyperspace: Closing hyper-threading side channels on sgx with contrived data races},
  author={Chen, Guoxing and Wang, Wenhao and Chen, Tianyu and Chen, Sanchuan and Zhang, Yinqian and Wang, XiaoFeng and Lai, Ten-Hwang and Lin, Dongdai},
  booktitle={2018 IEEE Symposium on Security and Privacy (SP)},
  pages={178--194},
  year={2018},
  organization={IEEE}
}

@inproceedings{marazzi2022protrr,
  title={Protrr: Principled yet optimal in-dram target row refresh},
  author={Marazzi, Michele and Jattke, Patrick and Solt, Flavien and Razavi, Kaveh},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={735--753},
  year={2022},
  organization={IEEE}
}

@inproceedings{frigo2020trrespass,
  title={TRRespass: Exploiting the many sides of target row refresh},
  author={Frigo, Pietro and Vannacc, Emanuele and Hassan, Hasan and Van Der Veen, Victor and Mutlu, Onur and Giuffrida, Cristiano and Bos, Herbert and Razavi, Kaveh},
  booktitle={2020 IEEE Symposium on Security and Privacy (SP)},
  pages={747--762},
  year={2020},
  organization={IEEE}
}

@inproceedings{kim2023kill,
  title={How to Kill the Second Bird with One ECC: The Pursuit of Row Hammer Resilient DRAM},
  author={Kim, Michael Jaemin and Wi, Minbok and Park, Jaehyun and Ko, Seoyoung and Choi, Jaeyoung and Nam, Hwayoung and Kim, Nam Sung and Ahn, Jung Ho and Lee, Eojin},
  booktitle={Proceedings of the 56th Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={986--1001},
  year={2023}
}

@inproceedings{dessouky2020hybcache,
  title={$\{$HybCache$\}$: Hybrid $\{$Side-Channel-Resilient$\}$ caches for trusted execution environments},
  author={Dessouky, Ghada and Frassetto, Tommaso and Sadeghi, Ahmad-Reza},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={451--468},
  year={2020}
}

@article{godfrey2014preventing,
  title={Preventing cache-based side-channel attacks in a cloud environment},
  author={Godfrey, Michael and Zulkernine, Mohammad},
  journal={IEEE transactions on cloud computing},
  volume={2},
  number={4},
  pages={395--408},
  year={2014},
  publisher={IEEE}
}

@inproceedings{khasawneh2019safespec,
  title={Safespec: Banishing the spectre of a meltdown with leakage-free speculation},
  author={Khasawneh, Khaled N and Koruyeh, Esmaeil Mohammadian and Song, Chengyu and Evtyushkin, Dmitry and Ponomarev, Dmitry and Abu-Ghazaleh, Nael},
  booktitle={2019 56th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}
@inproceedings{lehman2016poisonivy,
  title={PoisonIvy: Safe speculation for secure memory},
  author={Lehman, Tamara Silbergleit and Hilton, Andrew D and Lee, Benjamin C},
  booktitle={2016 49th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={1--13},
  year={2016},
  organization={IEEE}
}

@inproceedings{yan2018invisispec,
  title={Invisispec: Making speculative execution invisible in the cache hierarchy},
  author={Yan, Mengjia and Choi, Jiho and Skarlatos, Dimitrios and Morrison, Adam and Fletcher, Christopher and Torrellas, Josep},
  booktitle={2018 51st Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={428--441},
  year={2018},
  organization={IEEE}
}

@inproceedings{shih2017t,
  title={T-SGX: Eradicating Controlled-Channel Attacks Against Enclave Programs.},
  author={Shih, Ming-Wei and Lee, Sangho and Kim, Taesoo and Peinado, Marcus},
  booktitle={NDSS},
  year={2017}
}

@inproceedings{zhou2016software,
  title={A software approach to defeating side channels in last-level caches},
  author={Zhou, Ziqiao and Reiter, Michael K and Zhang, Yinqian},
  booktitle={Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security},
  pages={871--882},
  year={2016}
}

@inproceedings{zhang2013duppel,
  title={D{\"u}ppel: Retrofitting commodity operating systems to mitigate cache side channels in the cloud},
  author={Zhang, Yinqian and Reiter, Michael K},
  booktitle={Proceedings of the 2013 ACM SIGSAC conference on Computer \& communications security},
  pages={827--838},
  year={2013}
}

@inproceedings{orenbach2017eleos,
  title={Eleos: ExitLess OS services for SGX enclaves},
  author={Orenbach, Meni and Lifshits, Pavel and Minkin, Marina and Silberstein, Mark},
  booktitle={Proceedings of the Twelfth European Conference on Computer Systems},
  pages={238--253},
  year={2017}
}

@inproceedings{chen2016remix,
  title={Remix: On-demand live randomization},
  author={Chen, Yue and Wang, Zhi and Whalley, David and Lu, Long},
  booktitle={Proceedings of the sixth ACM conference on data and application security and privacy},
  pages={50--61},
  year={2016}
}

@article{elatali2024cancellable,
  title={Cancellable Memory Requests: A transparent, lightweight Spectre mitigation},
  author={ElAtali, Hossam and Asokan, N},
  journal={arXiv preprint arXiv:2406.12110},
  year={2024}
}

@inproceedings{wang2020mitigating,
  title={Mitigating cache-based side-channel attacks through randomization: A comprehensive system and architecture level analysis},
  author={Wang, Han and Sayadi, Hossein and Mohsenin, Tinoosh and Zhao, Liang and Sasan, Avesta and Rafatirad, Setareh and Homayoun, Houman},
  booktitle={2020 Design, Automation \& Test in Europe Conference \& Exhibition (DATE)},
  pages={1414--1419},
  year={2020},
  organization={IEEE}
}

@inproceedings{dong2018shielding,
  title={Shielding Software From Privileged $\{$Side-Channel$\}$ Attacks},
  author={Dong, Xiaowan and Shen, Zhuojia and Criswell, John and Cox, Alan L and Dwarkadas, Sandhya},
  booktitle={27th USENIX Security Symposium (USENIX Security 18)},
  pages={1441--1458},
  year={2018}
}

@inproceedings{doychev2017rigorous,
  title={Rigorous analysis of software countermeasures against cache attacks},
  author={Doychev, Goran and K{\"o}pf, Boris},
  booktitle={Proceedings of the 38th ACM SIGPLAN Conference on Programming Language Design and Implementation},
  pages={406--421},
  year={2017}
}

@article{strackx2017heisenberg,
  title={The Heisenberg defense: Proactively defending SGX enclaves against page-table-based side-channel attacks},
  author={Strackx, Raoul and Piessens, Frank},
  journal={arXiv preprint arXiv:1712.08519},
  year={2017}
}

@inproceedings{ahmad2019obfuscuro,
  title={OBFUSCURO: A commodity obfuscation engine on Intel SGX},
  author={Ahmad, Adil and Joe, Byunggill and Xiao, Yuan and Zhang, Yinqian and Shin, Insik and Lee, Byoungyoung},
  booktitle={Network and Distributed System Security Symposium},
  year={2019}
}

@inproceedings{crane2015thwarting,
  title={Thwarting cache side-channel attacks through dynamic software diversity.},
  author={Crane, Stephen and Homescu, Andrei and Brunthaler, Stefan and Larsen, Per and Franz, Michael},
  booktitle={NDSS},
  pages={8--11},
  year={2015}
}

@inproceedings{li2020dlfix,
  title={Dlfix: Context-based code transformation learning for automated program repair},
  author={Li, Yi and Wang, Shaohua and Nguyen, Tien N},
  booktitle={Proceedings of the ACM/IEEE 42nd international conference on software engineering},
  pages={602--614},
  year={2020}
}

@article{li2024p,
  title={P refender: A Prefetching Defender against Cache Side Channel Attacks as A Pretender},
  author={Li, Luyi and Huang, Jiayi and Feng, Lang and Wang, Zhongfeng},
  journal={IEEE Transactions on Computers},
  year={2024},
  publisher={IEEE}
}

@inproceedings{palit2019mitigating,
  title={Mitigating data leakage by protecting memory-resident sensitive data},
  author={Palit, Tapti and Monrose, Fabian and Polychronakis, Michalis},
  booktitle={Proceedings of the 35th Annual Computer Security Applications Conference},
  pages={598--611},
  year={2019}
}

@article{brasser2017dr,
  title={DR. SGX: hardening SGX enclaves against cache attacks with data location randomization},
  author={Brasser, Ferdinand and Capkun, Srdjan and Dmitrienko, Alexandra and Frassetto, Tommaso and Kostiainen, Kari and Sadeghi, Ahmad-Reza},
  journal={arXiv preprint arXiv:1709.09917},
  year={2017}
}

@inproceedings{kim2012stealthmem,
  title={$\{$STEALTHMEM$\}$:$\{$System-Level$\}$ protection against $\{$Cache-Based$\}$ side channel attacks in the cloud},
  author={Kim, Taesoo and Peinado, Marcus and Mainar-Ruiz, Gloria},
  booktitle={21st USENIX Security Symposium (USENIX Security 12)},
  pages={189--204},
  year={2012}
}

@inproceedings{tan2023ptstore,
  title={PTStore: Lightweight Architectural Support for Page Table Isolation},
  author={Tan, Wende and Chen, Yangyu and Li, Yuan and Liu, Ying and Wu, Jianping and Ding, Yu and Zhang, Chao},
  booktitle={2023 60th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--6},
  year={2023},
  organization={IEEE}
}

@inproceedings{rane2015raccoon,
  title={Raccoon: Closing digital $\{$Side-Channels$\}$ through obfuscated execution},
  author={Rane, Ashay and Lin, Calvin and Tiwari, Mohit},
  booktitle={24th USENIX Security Symposium (USENIX Security 15)},
  pages={431--446},
  year={2015}
}

@inproceedings{goubin2002refined,
  title={A refined power-analysis attack on elliptic curve cryptosystems},
  author={Goubin, Louis},
  booktitle={Public Key Cryptography—PKC 2003: 6th International Workshop on Practice and Theory in Public Key Cryptography Miami, FL, USA, January 6--8, 2003 Proceedings 6},
  pages={199--211},
  year={2002},
  organization={Springer}
}

@inproceedings{kocher1996timing,
  title={Timing attacks on implementations of Diffie-Hellman, RSA, DSS, and other systems},
  author={Kocher, Paul C},
  booktitle={Advances in Cryptology—CRYPTO’96: 16th Annual International Cryptology Conference Santa Barbara, California, USA August 18--22, 1996 Proceedings 16},
  pages={104--113},
  year={1996},
  organization={Springer}
}

@article{jiang2020mempoline,
  title={Mempoline: Mitigating memory-based side-channel attacks through memory access obfuscation},
  author={Jiang, Zhen Hang and Fei, Yunsi and Ding, Aidong Adam and Wahl, Thomas},
  journal={Cryptology ePrint Archive},
  year={2020}
}

@article{morel2023code,
  title={Code Polymorphism Meets Code Encryption: Confidentiality and Side-Channel Protection of Software Components},
  author={Morel, Lionel and Courouss{\'e}, Damien and Hiscock, Thomas},
  journal={Digital Threats: Research and Practice},
  volume={4},
  number={2},
  pages={1--27},
  year={2023},
  publisher={ACM New York, NY, USA}
}

@inproceedings{gentry2009fully,
  title={Fully homomorphic encryption using ideal lattices},
  author={Gentry, Craig},
  booktitle={Proceedings of the forty-first annual ACM symposium on Theory of computing},
  pages={169--178},
  year={2009}
}

@inproceedings{joye2002montgomery,
  title={The Montgomery powering ladder},
  author={Joye, Marc and Yen, Sung-Ming},
  booktitle={International workshop on cryptographic hardware and embedded systems},
  pages={291--302},
  year={2002},
  organization={Springer}
}

@inproceedings{wichelmann2023cipherfix,
  title={Cipherfix: Mitigating Ciphertext $\{$Side-Channel$\}$ Attacks in Software},
  author={Wichelmann, Jan and P{\"a}tschke, Anna and Wilke, Luca and Eisenbarth, Thomas},
  booktitle={32nd USENIX Security Symposium (USENIX Security 23)},
  pages={6789--6806},
  year={2023}
}

@inproceedings{wu2018eliminating,
  title={Eliminating timing side-channel leaks using program repair},
  author={Wu, Meng and Guo, Shengjian and Schaumont, Patrick and Wang, Chao},
  booktitle={Proceedings of the 27th ACM SIGSOFT International Symposium on Software Testing and Analysis},
  pages={15--26},
  year={2018}
}

@inproceedings{dziembowski2008leakage,
  title={Leakage-resilient cryptography},
  author={Dziembowski, Stefan and Pietrzak, Krzysztof},
  booktitle={2008 49th Annual IEEE Symposium on Foundations of Computer Science},
  pages={293--302},
  year={2008},
  organization={IEEE}
}

@article{unterluggauer2019meas,
  title={MEAS: Memory encryption and authentication secure against side-channel attacks},
  author={Unterluggauer, Thomas and Werner, Mario and Mangard, Stefan},
  journal={Journal of cryptographic engineering},
  volume={9},
  pages={137--158},
  year={2019},
  publisher={Springer}
}

@inproceedings{tsoupidi2023securing,
  title={Securing optimized code against power side channels},
  author={Tsoupidi, Rodothea Myrsini and Lozano, Roberto Casta{\~n}eda and Troubitsyna, Elena and Papadimitratos, Panagiotis},
  booktitle={2023 IEEE 36th Computer Security Foundations Symposium (CSF)},
  pages={340--355},
  year={2023},
  organization={IEEE}
}

@article{domnitser2012non,
  title={Non-monopolizable caches: Low-complexity mitigation of cache side channel attacks},
  author={Domnitser, Leonid and Jaleel, Aamer and Loew, Jason and Abu-Ghazaleh, Nael and Ponomarev, Dmitry},
  journal={ACM Transactions on Architecture and Code Optimization (TACO)},
  volume={8},
  number={4},
  pages={1--21},
  year={2012},
  publisher={ACM New York, NY, USA}
}

@inproceedings{fiore2018optimal,
  title={Optimal partitioning of LLC in CAT-enabled CPUs to prevent side-channel attacks},
  author={Fiore, Ugo and Florea, Adrian and Gellert, Arpad and Vintan, Lucian and Zanetti, Paolo},
  booktitle={International Symposium on Cyberspace Safety and Security},
  pages={115--123},
  year={2018},
  organization={Springer}
}

@article{dessouky2021chunked,
  title={Chunked-cache: On-demand and scalable cache isolation for security architectures},
  author={Dessouky, Ghada and Gruler, Alexander and Mahmoody, Pouya and Sadeghi, Ahmad-Reza and Stapf, Emmanuel},
  journal={arXiv preprint arXiv:2110.08139},
  year={2021}
}

@article{song2022remapped,
  title={Remapped Cache Layout: Thwarting Cache-Based Side-Channel Attacks with a Hardware Defense},
  author={Song, Wei and Hou, Rui and Liu, Peng and Li, Xiaoxin and Li, Peinan and Zhao, Lutan and Fu, Xiaofei and Sun, Yifei and Meng, Dan},
  journal={arXiv preprint arXiv:2211.06056},
  year={2022}
}

@inproceedings{sprabery2018scheduling,
  title={Scheduling, isolation, and cache allocation: A side-channel defense},
  author={Sprabery, Read and Evchenko, Konstantin and Raj, Abhilash and Bobba, Rakesh B and Mohan, Sibin and Campbell, Roy},
  booktitle={2018 IEEE International Conference on Cloud Engineering (IC2E)},
  pages={34--40},
  year={2018},
  organization={IEEE}
}

@inproceedings{varadarajan2014scheduler,
  title={Scheduler-based defenses against $\{$Cross-VM$\}$ side-channels},
  author={Varadarajan, Venkatanathan and Ristenpart, Thomas and Swift, Michael},
  booktitle={23rd USENIX security symposium (USENIX security 14)},
  pages={687--702},
  year={2014}
}

@inproceedings{oleksenko2018varys,
  title={Varys: Protecting $\{$SGX$\}$ Enclaves from Practical $\{$Side-Channel$\}$ Attacks},
  author={Oleksenko, Oleksii and Trach, Bohdan and Krahn, Robert and Silberstein, Mark and Fetzer, Christof},
  booktitle={2018 Usenix Annual Technical Conference (USENIX ATC 18)},
  pages={227--240},
  year={2018}
}

@inproceedings{deutsch2022dagguise,
  title={DAGguise: mitigating memory timing side channels},
  author={Deutsch, Peter W and Yang, Yuheng and Bourgeat, Thomas and Drean, Jules and Emer, Joel S and Yan, Mengjia},
  booktitle={Proceedings of the 27th ACM International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={329--343},
  year={2022}
}

@article{geng2024new,
  title={A New Secure Memory System for Efficient Data Protection and Access Pattern Obfuscation},
  author={Geng, Haoran and Che, Yuezhi and Dingler, Aaron and Niemier, Michael and Hu, Xiaobo Sharon},
  journal={arXiv preprint arXiv:2402.15824},
  year={2024}
}

@article{doychev2015cacheaudit,
  title={Cacheaudit: A tool for the static analysis of cache side channels},
  author={Doychev, Goran and K{\"o}pf, Boris and Mauborgne, Laurent and Reineke, Jan},
  journal={ACM Transactions on information and system security (TISSEC)},
  volume={18},
  number={1},
  pages={1--32},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@inproceedings{brotzman2019casym,
  title={CaSym: Cache aware symbolic execution for side channel detection and mitigation},
  author={Brotzman, Robert and Liu, Shen and Zhang, Danfeng and Tan, Gang and Kandemir, Mahmut},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={505--521},
  year={2019},
  organization={IEEE}
}

@article{chiappetta2016real,
  title={Real time detection of cache-based side-channel attacks using hardware performance counters},
  author={Chiappetta, Marco and Savas, Erkay and Yilmaz, Cemal},
  journal={Applied Soft Computing},
  volume={49},
  pages={1162--1174},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{wang2017cached,
  title={$\{$CacheD$\}$: Identifying $\{$Cache-Based$\}$ timing channels in production software},
  author={Wang, Shuai and Wang, Pei and Liu, Xiao and Zhang, Danfeng and Wu, Dinghao},
  booktitle={26th USENIX security symposium (USENIX security 17)},
  pages={235--252},
  year={2017}
}

@inproceedings{wu2022predator,
  title={PREDATOR: A Cache Side-Channel Attack Detector Based on Precise Event Monitoring},
  author={Wu, Minjun and McCamant, Stephen and Yew, Pen-Chung and Zhai, Antonia},
  booktitle={2022 IEEE International Symposium on Secure and Private Execution Environment Design (SEED)},
  pages={25--36},
  year={2022},
  organization={IEEE}
}

@article{kim2023deep,
  title={Deep learning based detection for multiple cache side-channel attacks},
  author={Kim, Hodong and Hahn, Changhee and Kim, Hyunwoo J and Shin, Youngjoo and Hur, Junbeom},
  journal={IEEE Transactions on Information Forensics and Security},
  year={2023},
  publisher={IEEE}
}

@inproceedings{wang2020scarf,
  title={Scarf: Detecting side-channel attacks at real-time using low-level hardware features},
  author={Wang, Han and Sayadi, Hossein and Rafatirad, Setareh and Sasan, Avesta and Homayoun, Houman},
  booktitle={2020 IEEE 26th International Symposium on On-Line Testing and Robust System Design (IOLTS)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@article{raj2017keep,
  title={Keep the PokerFace on! Thwarting cache side channel attacks by memory bus monitoring and cache obfuscation},
  author={Raj, Arun and Dharanipragada, Janakiram},
  journal={Journal of Cloud Computing},
  volume={6},
  pages={1--14},
  year={2017},
  publisher={Springer}
}

@article{carna2023fight,
  title={Fight hardware with hardware: Systemwide detection and mitigation of side-channel attacks using performance counters},
  author={Carn{\`a}, Stefano and Ferracci, Serena and Quaglia, Francesco and Pellegrini, Alessandro},
  journal={Digital Threats: Research and Practice},
  volume={4},
  number={1},
  pages={1--24},
  year={2023},
  publisher={ACM New York, NY}
}

@article{sangeetha2021optimistic,
  title={An optimistic technique to detect cache based side channel attacks in cloud},
  author={Sangeetha, G and Sumathi, G},
  journal={Peer-to-Peer networking and Applications},
  volume={14},
  number={4},
  pages={2473--2486},
  year={2021},
  publisher={Springer}
}

@inproceedings{osvik2006cache,
  title={Cache attacks and countermeasures: the case of AES},
  author={Osvik, Dag Arne and Shamir, Adi and Tromer, Eran},
  booktitle={Topics in Cryptology--CT-RSA 2006: The Cryptographers’ Track at the RSA Conference 2006, San Jose, CA, USA, February 13-17, 2005. Proceedings},
  pages={1--20},
  year={2006},
  organization={Springer}
}

@article{kiriansky2018speculative,
  title={Speculative buffer overflows: Attacks and defenses},
  author={Kiriansky, Vladimir and Waldspurger, Carl},
  journal={arXiv preprint arXiv:1807.03757},
  year={2018}
}

@techreport{intel_retpoline_2018,
  title        = {Retpoline: A Branch Target Injection Mitigation},
  author       = {{Intel Corporation}},
  year         = 2018,
  month        = jun,
  url          = {https://www.intel.com/content/dam/develop/external/us/en/documents/retpoline-a-branch-target-injection-mitigation.pdf},
  institution  = {Intel Corporation},
  type         = {White Paper},
  number       = {337131-003}
}

@book{jacob2010memory,
  title={Memory systems: cache, DRAM, disk},
  author={Jacob, Bruce and Wang, David and Ng, Spencer},
  year={2010},
  publisher={Morgan Kaufmann}
}

@article{barham2003xen,
  title={Xen and the art of virtualization},
  author={Barham, Paul and Dragovic, Boris and Fraser, Keir and Hand, Steven and Harris, Tim and Ho, Alex and Neugebauer, Rolf and Pratt, Ian and Warfield, Andrew},
  journal={ACM SIGOPS operating systems review},
  volume={37},
  number={5},
  pages={164--177},
  year={2003},
  publisher={ACM New York, NY, USA}
}

@inproceedings{bosman2016dedup,
  title={Dedup est machina: Memory deduplication as an advanced exploitation vector},
  author={Bosman, Erik and Razavi, Kaveh and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={2016 IEEE symposium on security and privacy (SP)},
  pages={987--1004},
  year={2016},
  organization={IEEE}
}

@inproceedings{zhang2012cross,
  title={Cross-VM side channels and their use to extract private keys},
  author={Zhang, Yinqian and Juels, Ari and Reiter, Michael K and Ristenpart, Thomas},
  booktitle={Proceedings of the 2012 ACM conference on Computer and communications security},
  pages={305--316},
  year={2012}
}

@article{lyu2018survey,
  title={A survey of side-channel attacks on caches and countermeasures},
  author={Lyu, Yangdi and Mishra, Prabhat},
  journal={Journal of Hardware and Systems Security},
  volume={2},
  pages={33--50},
  year={2018},
  publisher={Springer}
}

@article{zhang2014cache,
  title={Cache-based Side-Channel Attacks in Multi-Tenant Public Clouds and Their Countermeasures},
  author={Zhang, Yinqian},
  year={2014},
  publisher={University of North Carolina at Chapel Hill Graduate School}
}

@article{lou2021survey,
  title={A survey of microarchitectural side-channel vulnerabilities, attacks, and defenses in cryptography},
  author={Lou, Xiaoxuan and Zhang, Tianwei and Jiang, Jun and Zhang, Yinqian},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--37},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@inproceedings{canella2019systematic,
  title={A systematic evaluation of transient execution attacks and defenses},
  author={Canella, Claudio and Van Bulck, Jo and Schwarz, Michael and Lipp, Moritz and Von Berg, Benjamin and Ortner, Philipp and Piessens, Frank and Evtyushkin, Dmitry and Gruss, Daniel},
  booktitle={28th USENIX Security Symposium (USENIX Security 19)},
  pages={249--266},
  year={2019}
}

@inproceedings{gruss2018another,
  title={Another flip in the wall of rowhammer defenses},
  author={Gruss, Daniel and Lipp, Moritz and Schwarz, Michael and Genkin, Daniel and Juffinger, Jonas and O'Connell, Sioli and Schoechl, Wolfgang and Yarom, Yuval},
  booktitle={2018 IEEE Symposium on Security and Privacy (SP)},
  pages={245--261},
  year={2018},
  organization={IEEE}
}

@inproceedings{kim2020gpu,
  title={GPU side-channel attacks are everywhere: A survey},
  author={Kim, Taehun and Shin, Youngjoo},
  booktitle={2020 IEEE International Conference on Consumer Electronics-Asia (ICCE-Asia)},
  pages={1--4},
  year={2020},
  organization={IEEE}
}

@article{szefer2019survey,
  title={Survey of microarchitectural side and covert channels, attacks, and defenses},
  author={Szefer, Jakub},
  journal={Journal of Hardware and Systems Security},
  volume={3},
  number={3},
  pages={219--234},
  year={2019},
  publisher={Springer}
}

@article{lou2021survey,
  title={A survey of microarchitectural side-channel vulnerabilities, attacks, and defenses in cryptography},
  author={Lou, Xiaoxuan and Zhang, Tianwei and Jiang, Jun and Zhang, Yinqian},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--37},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{lungu2024gpu,
  title={GPU Side-Channel Attack Classification for Targeted Secure Shader Mitigation},
  author={Lungu, Nelson and Patra, Sudhansu Shekhar and Mishra, Manoj Ranjan and Dash, Bibhuti Bhusan and Sasmal, Gopal Charan and Pattnayak, Parthasarathi and Singh, Satyendr and Gourisaria, Mahendra Kumar},
  journal={SN Computer Science},
  volume={5},
  number={8},
  pages={1--23},
  year={2024},
  publisher={Springer}
}

@article{wang2023side,
  title={Side-channel attack analysis on in-memory computing architectures},
  author={Wang, Ziyu and Meng, Fan-hsuan and Park, Yongmo and Eshraghian, Jason K and Lu, Wei D},
  journal={IEEE Transactions on Emerging Topics in Computing},
  volume={12},
  number={1},
  pages={109--121},
  year={2023},
  publisher={IEEE}
}

@article{pulkit2023survey,
  title={A Survey of Side-Channel Attacks in Context of Cache--Taxonomies, Analysis and Mitigation},
  author={Pulkit, Ankit and Naval, Smita and Laxmi, Vijay},
  journal={arXiv preprint arXiv:2312.11094},
  year={2023}
}

@inproceedings{kwong2023checking,
  title={Checking Passwords on Leaky Computers: A Side Channel Analysis of Chrome's Password Leak Detect Protocol},
  author={Kwong, Andrew and Wang, Walter and Kim, Jason and Berger, Jonathan and Genkin, Daniel and Ronen, Eyal and Shacham, Hovav and Wahby, Riad and Yarom, Yuval},
  booktitle={32nd USENIX Security Symposium (USENIX Security 23)},
  pages={7107--7124},
  year={2023}
}

@inproceedings{wang2017side,
  title={Side-channel attacks on shared search indexes},
  author={Wang, Liang and Grubbs, Paul and Lu, Jiahui and Bindschaedler, Vincent and Cash, David and Ristenpart, Thomas},
  booktitle={2017 IEEE Symposium on Security and Privacy (SP)},
  pages={673--692},
  year={2017},
  organization={IEEE}
}

@article{naghibijouybari2019side,
  title={Side channel attacks on gpus},
  author={Naghibijouybari, Hoda and Neupane, Ajaya and Qian, Zhiyun and Abu-Ghazaleh, Nael},
  journal={IEEE Transactions on Dependable and Secure Computing},
  volume={18},
  number={4},
  pages={1950--1961},
  year={2019},
  publisher={IEEE}
}

@inproceedings{unterluggauer2016exploiting,
  title={Exploiting the physical disparity: Side-channel attacks on memory encryption},
  author={Unterluggauer, Thomas and Mangard, Stefan},
  booktitle={Constructive Side-Channel Analysis and Secure Design: 7th International Workshop, COSADE 2016, Graz, Austria, April 14-15, 2016, Revised Selected Papers 7},
  pages={3--18},
  year={2016},
  organization={Springer}
}

@inproceedings{lipp2021platypus,
  title={PLATYPUS: Software-based power side-channel attacks on x86},
  author={Lipp, Moritz and Kogler, Andreas and Oswald, David and Schwarz, Michael and Easdon, Catherine and Canella, Claudio and Gruss, Daniel},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={355--371},
  year={2021},
  organization={IEEE}
}

@article{alahmadi2022cyber,
  title={Cyber-security threats and side-channel attacks for digital agriculture},
  author={Alahmadi, Adel N and Rehman, Saeed Ur and Alhazmi, Husain S and Glynn, David G and Shoaib, Hatoon and Sol{\'e}, Patrick},
  journal={Sensors},
  volume={22},
  number={9},
  pages={3520},
  year={2022},
  publisher={MDPI}
}

@inproceedings{bazm2017side,
  title={Side-channels beyond the cloud edge: New isolation threats and solutions},
  author={Bazm, Mohammad-Mahdi and Lacoste, Marc and S{\"u}dholt, Mario and Menaud, Jean-Marc},
  booktitle={2017 1st Cyber Security in Networking Conference (CSNet)},
  pages={1--8},
  year={2017},
  organization={IEEE}
}

@article{mendez2021physical,
  title={Physical side-channel attacks on embedded neural networks: A survey},
  author={M{\'e}ndez Real, Maria and Salvador, Ruben},
  journal={Applied Sciences},
  volume={11},
  number={15},
  pages={6790},
  year={2021},
  publisher={MDPI}
}

@article{tsoupidi2023thwarting,
  title={Thwarting code-reuse and side-channel attacks in embedded systems},
  author={Tsoupidi, Rodothea Myrsini and Troubitsyna, Elena and Papadimitratos, Panagiotis},
  journal={Computers \& Security},
  volume={133},
  pages={103405},
  year={2023},
  publisher={Elsevier}
}

@article{fournaris2017exploiting,
  title={Exploiting hardware vulnerabilities to attack embedded system devices: A survey of potent microarchitectural attacks},
  author={Fournaris, Apostolos P and Pocero Fraile, Lidia and Koufopavlou, Odysseas},
  journal={Electronics},
  volume={6},
  number={3},
  pages={52},
  year={2017},
  publisher={MDPI}
}

@inproceedings{abrishamchi2017side,
  title={Side channel attacks on smart home systems: A short overview},
  author={Abrishamchi, Mohammad Ali Nassiri and Abdullah, Abdul Hanan and Cheok, Adrian David and Bielawski, Kevin S},
  booktitle={IECON 2017-43rd Annual Conference of the IEEE Industrial Electronics Society},
  pages={8144--8149},
  year={2017},
  organization={IEEE}
}

@inproceedings{karimi2018timing,
  title={A timing side-channel attack on a mobile gpu},
  author={Karimi, Elmira and Jiang, Zhen Hang and Fei, Yunsi and Kaeli, David},
  booktitle={2018 IEEE 36th International Conference on Computer Design (ICCD)},
  pages={67--74},
  year={2018},
  organization={IEEE}
}

@article{ahmed2024deep,
  title={Deep Learning Based Side-Channel Attack Detection for Mobile Devices Security in 5G Networks},
  author={Ahmed, Amjed A and Hasan, Mohammad Kamrul and Alqahtani, Ali and Islam, Shayla and Pandey, Bishwajeet and Rzayeva, Leila and Abbas, Huda Saleh and Aman, Azana Hafizah Mohd and Alqahtani, Nayef},
  journal={Tsinghua Science and Technology},
  volume={30},
  number={3},
  pages={1012--1026},
  year={2024},
  publisher={TUP}
}

@article{kong2012architecting,
  title={Architecting against software cache-based side-channel attacks},
  author={Kong, Jingfei and Aciicmez, Onur and Seifert, Jean-Pierre and Zhou, Huiyang},
  journal={IEEE Transactions on Computers},
  volume={62},
  number={7},
  pages={1276--1288},
  year={2012},
  publisher={IEEE}
}

@article{agredo2024inferring,
  title={Inferring TLB Configuration with Performance Tools},
  author={Agredo, Cristian and Langehaug, Tor J and Graham, Scott R},
  journal={Journal of Cybersecurity and Privacy},
  volume={4},
  number={4},
  pages={951--971},
  year={2024},
  publisher={MDPI}
}

@article{olmos2024protecting,
  title={Protecting cryptographic code against Spectre-RSB (and, in fact, all known Spectre variants)},
  author={Olmos, Santiago Arranz and Barthe, Gilles and Chuengsatiansup, Chitchanok and Gr{\'e}goire, Benjamin and Laporte, Vincent and Oliveira, Tiago and Schwabe, Peter and Yarom, Yuval and Zhang, Zhiyuan},
  year={2024}
}

@inproceedings{maisuradze2018ret2spec,
  title={ret2spec: Speculative execution using return stack buffers},
  author={Maisuradze, Giorgi and Rossow, Christian},
  booktitle={Proceedings of the 2018 ACM SIGSAC Conference on Computer and Communications Security},
  pages={2109--2122},
  year={2018}
}

@inproceedings{chowdhuryy2020branchspec,
  title={Branchspec: Information leakage attacks exploiting speculative branch instruction executions},
  author={Chowdhuryy, Md Hafizul Islam and Liu, Hang and Yao, Fan},
  booktitle={2020 IEEE 38th International Conference on Computer Design (ICCD)},
  pages={529--536},
  year={2020},
  organization={IEEE}
}

@inproceedings{wikner2024breaking,
  title={Breaking the Barrier: Post-Barrier Spectre Attacks},
  author={Wikner, Johannes and Razavi, Kaveh},
  booktitle={2025 IEEE Symposium on Security and Privacy (SP)},
  pages={89--89},
  year={2024},
  organization={IEEE Computer Society}
}

@article{kimslap,
  title={SLAP: Data Speculation Attacks via Load Address Prediction on Apple Silicon},
  author={Kim, Jason and Genkin, Daniel and Yarom, Yuval}
}

@inproceedings{kim2019high,
  title={High efficiency, low-noise meltdown attack by using a return stack buffer},
  author={Kim, TaeHyun and Shin, Youngjoo},
  booktitle={Proceedings of the 2019 ACM Asia Conference on Computer and Communications Security},
  pages={688--690},
  year={2019}
}

@inproceedings{koschel2020tagbleed,
  title={TagBleed: Breaking KASLR on the isolated kernel address space using tagged TLBs},
  author={Koschel, Jakob and Giuffrida, Cristiano and Bos, Herbert and Razavi, Kaveh},
  booktitle={2020 IEEE European Symposium on Security and Privacy (EuroS\&P)},
  pages={309--321},
  year={2020},
  organization={IEEE}
}

@phdthesis{irazoqui2017cross,
  title={Cross-core microarchitectural side channel attacks and countermeasures},
  author={Irazoqui, Gorka},
  year={2017},
  school={PhD thesis (Northeastern University, 2017)}
}

@inproceedings{lipp2022amd,
  title={$\{$AMD$\}$ prefetch attacks through power and time},
  author={Lipp, Moritz and Gruss, Daniel and Schwarz, Michael},
  booktitle={31st USENIX Security Symposium (USENIX Security 22)},
  pages={643--660},
  year={2022}
}

@book{chen2019exploitable,
  title={Exploitable Hardware Features and Vulnerabilities Enhanced Side-Channel Attacks on Intel SGX and Their Countermeasures},
  author={Chen, Guoxing},
  year={2019},
  publisher={The Ohio State University}
}

@phdthesis{ferracci2019detecting,
  title={Detecting cache-based side channel attacks using hardware performance counters},
  author={Ferracci, Serena},
  year={2019},
  school={Sapienza, University of Rome}
}

@inproceedings{guan2015protecting,
  title={Protecting private keys against memory disclosure attacks using hardware transactional memory},
  author={Guan, Le and Lin, Jingqiang and Luo, Bo and Jing, Jiwu and Wang, Jing},
  booktitle={2015 IEEE Symposium on Security and Privacy},
  pages={3--19},
  year={2015},
  organization={IEEE}
}

@inproceedings{van2017revanc,
  title={RevAnC: A framework for reverse engineering hardware page table caches},
  author={Van Schaik, Stephan and Razavi, Kaveh and Gras, Ben and Bos, Herbert and Giuffrida, Cristiano},
  booktitle={Proceedings of the 10th European Workshop on Systems Security},
  pages={1--6},
  year={2017}
}

@article{zhao2024you,
  title={YOU SHARE, YOU LEAK: PRACTICAL SIDE-CHANNEL ATTACKS AND DEFENSES IN MODERN CLOUDS},
  author={ZHAO, ZIRUI},
  year={2024}
}

@inproceedings{kim2020revisiting,
  title={Revisiting rowhammer: An experimental analysis of modern dram devices and mitigation techniques},
  author={Kim, Jeremie S and Patel, Minesh and Ya{\u{g}}l{\i}k{\c{c}}{\i}, A Giray and Hassan, Hasan and Azizi, Roknoddin and Orosa, Lois and Mutlu, Onur},
  booktitle={2020 ACM/IEEE 47th Annual International Symposium on Computer Architecture (ISCA)},
  pages={638--651},
  year={2020},
  organization={IEEE}
}

@article{zhang2022implicit,
  title={Implicit hammer: cross-privilege-boundary Rowhammer through implicit accesses},
  author={Zhang, Zhi and He, Wei and Cheng, Yueqiang and Wang, Wenhao and Gao, Yansong and Liu, Dongxi and Li, Kang and Nepal, Surya and Fu, Anmin and Zou, Yi},
  journal={IEEE Transactions on Dependable and Secure Computing},
  volume={20},
  number={5},
  pages={3716--3733},
  year={2022},
  publisher={IEEE}
}

@inproceedings{aga2017good,
  title={When good protections go bad: Exploiting anti-DoS measures to accelerate Rowhammer attacks},
  author={Aga, Misiker Tadesse and Aweke, Zelalem Birhanu and Austin, Todd},
  booktitle={2017 IEEE International Symposium on Hardware Oriented Security and Trust (HOST)},
  pages={8--13},
  year={2017},
  organization={IEEE}
}

@inproceedings{vano2018slicedup,
  title={Slicedup: a tenant-aware memory deduplication for cloud computing},
  author={Van{\'o}-Garc{\i}a, Fernando and Marco-Gisbert, Hector},
  booktitle={UBICOMM International Conference on Mobile Ubiquitous Computing, Systems, Services and Technologies, UBICOMM},
  pages={15--20},
  year={2018}
}

@phdthesis{maurice2015information,
  title={Information leakage on shared hardware: evolutions in recent hardware and applications to virtualization},
  author={Maurice, Clementine},
  year={2015},
  school={T{\'e}l{\'e}com ParisTech}
}
